Spectral Robustness for Correlation Clustering Reconstruction in Semi-Adversarial Models

Correlation Clustering is an important clustering problem with many applications. We study the reconstruction version of this problem in which one is seeking to reconstruct a latent clustering that has been corrupted by random noise and adversarial modifications. Concerning the latter, there is a standard "post-adversarial" model in the literature, in which adversarial modifications come after the noise. Here, we introduce and analyse a "pre-adversarial" model in which adversarial modifications come before the noise. Given an input coming from such a semi-adversarial generative model, the goal is to reconstruct almost perfectly and with high probability the latent clustering. We focus on the case where the hidden clusters have nearly equal size and show the following. In the pre-adversarial setting, spectral algorithms are optimal, in the sense that they reconstruct all the way to the information-theoretic threshold beyond which no reconstruction is possible. This is in contrast to the post-adversarial setting, in which their ability to restore the hidden clusters stops before the threshold, but the gap is optimally filled by SDP-based algorithms. These results highlight a heretofore unknown robustness of spectral algorithms, showing them less brittle than previously thought.

==> algo-k2-old.tex <==
\section{Recovering Two Hidden Clusters}\label{sec:k2}
For sake of the exposition, we first deal with the case of $k=2$ clusters, each of size $\nicefrac{n}{2}$. Having more clusters introduces additional technical complications that are dealt with separately. 
We analyse the pre-adversary first followed by the post-adversary.

First, notice that the input matrix $M$, in this setting, has rank $1$. Thus, its eigenspace for the eigenvalue $0$ has dimension $n-1$ by the Dimension Theorem for vector spaces. The other eigenvalue of $M$ is $n$, with corresponding unitary eigenvector $\bm{v}:=\frac{1}{\sqrt{n}}(\bm{f}_1 - \bm{f}_2)$, where $\bm{f}_i$ is the vector with $1$'s in the positions corresponding to the elements of the $i$\textsuperscript{th} cluster, and $0$ everywhere else. The key of our reconstruction algorithms is to approximately recover $\bm{v}$, because it contains all the needed information to reconstruct the original clusters.

\subsection{Spectral methods can cope with the pre-adversary}
Let 
\begin{equation}\label{preadv-params}
    \epsilon = \omega(n^{-1/2}) \; \; \;  \mbox{and} \; \; \; B=o(n^2).
\end{equation}
Recall that in this regime first the pre-adversary swaps $B$ entries of the original matrix $M$, giving rise to a matrix $M'$. Then, $M'$ is modified by random noise by swapping every entry with probability $1/2-\epsilon$. The resulting matrix is denoted as $M''$.
As we show in Section~\ref{sec:infotheo}, if $\epsilon = o(n^{-1/2})$ or $B=\Omega(n^2)$ information-theoretic lower bounds kick in and no reconstruction is possible.
We begin with some useful facts about the norms of these matrices.

\begin{lemma}\label{preadv-first-ineq}
$\|M'-M\|_{op} \leq 2\sqrt{B} = o(n).$
\end{lemma}
\begin{proof}
Define $E:=M'-M$. By definition, $E$ has $B$ non-zero entries, each of which is either $-2$ or $2$. Therefore, $\|E\|_F = \sqrt{4B} = 2\sqrt{B}$. By Lemma~\ref{norms-ineq}, this implies that $\|E\|_{op} \leq  2\sqrt{B}$.
\end{proof}

\begin{lemma}\label{preadv-second-ineq}
$\Pr(\|M''-\mathbb{E}[M'']\|_{op} \geq 16 \sqrt{n}) \leq 2^{-4n}.$
\end{lemma}
\begin{proof}
First, notice that $\mathbb{E}[M''] = \left( \frac{1}{2} + \epsilon \right) M' + \left( \frac{1}{2} - \epsilon \right)(-M') = 2\epsilon \cdot M'$, so
$$M_{i,j}'' - \mathbb{E}[M_{i,j}''] := 
\begin{cases}
      (1-2\epsilon)M_{i,j}' & \text{w. pr. } \frac{1}{2} + \epsilon;\\
       -(1+2\epsilon)M_{i,j}' & \text{w. pr. } \frac{1}{2} - \epsilon.
    \end{cases}
$$
Thus $\frac{1}{1+2\epsilon}(M''-\mathbb{E}[M''])$ has all the elements bounded by $1$ in absolute value. Moreover, we can write it as the sum of its upper triangular part, name it $N$, and its lower triangular part, $N^T$: $\frac{1}{1+2\epsilon}(M''-\mathbb{E}[M'']) = N + N^T$. The matrix $N$ satisfies the hypothesis of Theorem~\ref{opnorm-random}, so $\Pr(\|N\|_{op} \geq 4 \cdot \sqrt{n}) \leq 2^{-4n}$. By the triangle inequality $\Pr(\|N+N^T\|_{op} \geq 8 \cdot \sqrt{n}) \leq \Pr(\|N\|_{op}+\|N^T\|_{op} \geq 8 \cdot \sqrt{n}) $. However, $\|N\|_{op} = \|N^T\|_{op}$, so $\Pr(\|N+N^T\|_{op} \geq 8 \cdot \sqrt{n}) = \Pr(\|N\|_{op} \geq 4 \cdot \sqrt{n}) \leq 2^{-4n}$. Finally, $\Pr(\|M''-\mathbb{E}[M'']\|_{op} \geq 16 \sqrt{n}) = \Pr((1+2\epsilon)\|N+N^T\|_{op} \geq 16 \sqrt{n}) \leq \Pr(\|N+N^T\|_{op} \geq 8 \cdot \sqrt{n}) \leq 2^{-4n}$ because $\epsilon \leq \nicefrac{1}{2}$.
\end{proof}

\begin{theorem}\label{preadv-displ}
With probability at least $1 -2^{-4n}=1-o(1)$,
$\|M''-2\epsilon \cdot M\|_{op} \leq 16 \sqrt{n} + 4\epsilon \cdot \sqrt{B} = o(\epsilon n).$
\end{theorem}
\begin{proof}
By the triangle inequality, $\|M''-2\epsilon \cdot M\|_{op} \leq \|M''-\mathbb{E}[M'']\|_{op} + \|\mathbb{E}[M'']-2\epsilon \cdot M\|_{op}$. First, by Lemma~\ref{preadv-second-ineq}, with high probability $\geq 1 -2^{-4n}=1-o(1)$, it holds $\|M''-\mathbb{E}[M'']\|_{op} \leq 16 \sqrt{n}$. Second, we have that $\mathbb{E}[M''] = 2\epsilon \cdot M'$, so $\|\mathbb{E}[M'']-2\epsilon \cdot M\|_{op} = 2\epsilon \cdot \|M'-M\|_{op}$. However, by Lemma~\ref{preadv-first-ineq}, it holds $\|M'-M\|_{op} \leq 2\sqrt{B}$. By putting everything together, we finally get that $\|M''-2\epsilon \cdot M\|_{op} \leq 16 \sqrt{n} + 4\epsilon \cdot \sqrt{B}$. Finally, we notice that $16 \sqrt{n} + 4\epsilon \cdot \sqrt{B} = o(\epsilon n)$ by Equation~\ref{preadv-params}.
\end{proof}

We now show that the principal eigenvector of $M''$ is very close to that of $M$, which encodes the latent clustering, paving the way to the use of  spectral algorithms. 

\begin{lemma}\label{spectral-preadv-2}
Let $\bm{v}$ and $\bm{v}''$ be the principal unitary eigenvectors of $M$ and $M''$, respectively. Then, with probability at least $1-2^{-4n} = 1-o(1)$,  
$$\|\bm{v} - \bm{v}''\| \leq \frac{8}{\epsilon \sqrt{n}} + \frac{2\sqrt{B}}{n} = o(1).$$
\end{lemma}
\begin{proof}
By what observed about the eigenvalues of $M$, $2\epsilon \cdot M$ is diagonalizable with eigenvalues $2\epsilon n$ and $0$. Thus, by Theorem~\ref{davis-kahan}, there is such a unitary eigenvector $\bm{v}$ for which
$\|\bm{v}\bm{v}^T - \bm{v}''(\bm{v}'')^T\|_F \leq \frac{\|M''-2\epsilon \cdot M\|_{op}}{2\epsilon n}$. First, it holds $\|\bm{v}\bm{v}^T - \bm{v}''(\bm{v}'')^T\|_F^2 = \sum_{i,j=1}^{n}{(\bm{v}_i\bm{v}_j-\bm{v}_i''\bm{v}_j'')^2} = 2 - 2\langle \bm{v},\bm{v}'' \rangle^2$. Second, by Theorem~\ref{preadv-displ}, with high probability $\geq 1 -2^{-4n}=1-o(1)$, it holds $\|M''-2\epsilon \cdot M\|_{op} \leq 16 \sqrt{n} + 4\epsilon \cdot \sqrt{B} = o(\epsilon n)$, so 
$$2 - 2\langle \bm{v},\bm{v}'' \rangle^2 \leq \left(\frac{16 \sqrt{n} + 4\epsilon \cdot \sqrt{B}}{2\epsilon n}\right)^2 = \left( \frac{8}{\epsilon \sqrt{n}} + \frac{2\sqrt{B}}{n} \right)^2 = o(1)$$
$$\Longrightarrow \langle \bm{v},\bm{v}'' \rangle \geq \sqrt{1 - \frac{1}{2} \cdot \left( \frac{8}{\epsilon \sqrt{n}} + \frac{2\sqrt{B}}{n} \right)^2} \geq 1 - \frac{1}{2} \cdot \left( \frac{8}{\epsilon \sqrt{n}} + \frac{2\sqrt{B}}{n} \right)^2 = 1 - o(1)$$
because $\sqrt{1-x} \geq 1-x$ for each $x \in [0,1]$. However, $\|\bm{v}-\bm{v}''\|^2 = 2 - 2\langle \bm{v},\bm{v}'' \rangle$, which implies that $$\|\bm{v} - \bm{v}''\|^2 \leq \left( \frac{8}{\epsilon \sqrt{n}} + \frac{2\sqrt{B}}{n} \right)^2 = o(1).\qedhere$$
\end{proof}

Lemma~\ref{spectral-preadv-2} implies that a straightforward application of the well-known power method  can recover the latent clusters almost perfectly (see \cite{golub1996matrix}).  This is spelled out in Algorithm~\ref{alg:preadv-2}.

\begin{algorithm}
\caption{Input: $M''$, $n$}
\label{alg:preadv-2}
\begin{algorithmic}[1]
\STATE $\mathcal{S}_1 \leftarrow \emptyset;\ \mathcal{S}_2 \leftarrow \emptyset$
\STATE Let $\bm{v}''$ be the eigenvector of the leading eigenvalue of $M''$ computed with the \power
\FOR{$i = 1,\dots,n$}
\IF{$\bm{v}''_i > 0$}
\STATE $\mathcal{S}_1 \leftarrow \mathcal{S}_1 \cup \{i\}$
\ELSE
\STATE $\mathcal{S}_2 \leftarrow \mathcal{S}_2 \cup \{i\}$
\ENDIF
\ENDFOR
\STATE \textbf{Return } $\{\mathcal{S}_1,\mathcal{S}_2\}$
\end{algorithmic}
\end{algorithm}

\begin{theorem}\label{preadv-2-works}
With probability $1-o(1)$, Algorithm~\ref{alg:preadv-2} correctly classifies $n-o(n)$ vertices, where the number of misclassified vertices is at most $ \nicefrac{128}{\epsilon^2} + \nicefrac{8B}{n} = o(n)$.
\end{theorem}
\begin{proof}
Let $\bm{v}$ be a unitary eigenvector of the largest eigenvalue of $M$ (or, equivalently, of $2\epsilon \cdot M$), and let $\bm{v}''$ be the unitary eigenvector of the largest eigenvalue of $M''$. By Lemma~\ref{spectral-preadv-2} we have that, with high probability $\geq 1-2^{-4n} = 1-o(1)$, it holds 
$$\|\bm{v} - \bm{v}''\| \leq \frac{8}{\epsilon \sqrt{n}} + \frac{2\sqrt{B}}{n} = o(1).$$
Now, unless we swap the clusters, we can write w.l.o.g. $\bm{v} = \frac{1}{\sqrt{n}}\bm{f}_1 - \frac{1}{\sqrt{n}}\bm{f}_2$, where $\bm{f}_i$ is the indicator vector of the $i^{th}$ cluster. Now, let $\mathcal{S}_{bad}:=\{i \in [n]: \bm{v}_i\bm{v}_i'' < 0\}$, i.e. the set of coordinates with swapped signs between $\bm{v}$ and $\bm{v}''$. Those correspond exactly to the misplaced vertices in Algorithm~\ref{alg:preadv-2}. However, if $i \in \mathcal{S}_{bad}$, by definition of $\bm{v}$, we have either $\bm{v}_i = \frac{1}{\sqrt{n}}$ and $\bm{v}_i'' \leq 0$ or $\bm{v}_i = - \frac{1}{\sqrt{n}}$ and $\bm{v}_i'' \geq 0$, implying that $|\bm{v}_i-\bm{v}_i''| \geq \frac{1}{\sqrt{n}}$. Thus,
$$\left(\frac{8}{\epsilon \sqrt{n}} + \frac{2\sqrt{B}}{n}\right)^2 \geq \|\bm{v} - \bm{v}''\|^2 \geq \sum_{i \in \mathcal{S}_{bad}}{|\bm{v}_i-\bm{v}_i''|^2} \geq \frac{|\mathcal{S}_{bad}|}{n},$$
implying that $|\mathcal{S}_{bad}| \leq n\left(\frac{8}{\epsilon \sqrt{n}} + \frac{2\sqrt{B}}{n}\right)^2 \leq n \left( \frac{128}{\epsilon^2 n} + \frac{8B}{n^2} \right)= \frac{128}{\epsilon^2} + \frac{8B}{n} =  o(n)$, where we used that $(a+b)^2 \leq 2(a^2 + b^2)$ for each $a, b \in \mathbb{R}$.
\end{proof}

Except for the invocation of the \power, the running time of Algorithm~\ref{alg:preadv-2} is linear in $n$. 
The running time of the \power\ depends on the ratio between the first eigenvalue and the gap between the first two eigenvalues of $M''$. 
This is $\approx 1$ because $\|M''-2\epsilon \cdot M\|_{op} \leq 16 \sqrt{n} + 4\epsilon \cdot \sqrt{B} = o(\epsilon n)$ with high probability by Theorem~\ref{preadv-displ}. And so this ratio is very close to the one of $M$, which is $1$. It follows by known facts about the \power\ that its running time is polynomial, and it computes a solution with negligible error.
 

\subsection{Dealing with the Post-Adversary}
Let us now consider the post-adversarial setting. We first show that the spectral algorithms, perhaps surprisingly, remain somewhat robust in the presence of a post-adversary. Their robustness is limited however, and unable to match the information-theoretic lower bounds we establish in Section~\ref{sec:infotheo}. Fortunately, the gap  can be filled thanks to an SDP-based approach that is optimal in this setting.

As before, we begin by proving a few useful facts about matrix norms of our matrices.
\begin{lemma}\label{postadv-first-ineq}
$\Pr(\|M'-\mathbb{E}[M']\|_{\inftone} \geq 16 n\sqrt{n}) \leq \Pr(\|M'-\mathbb{E}[M']\|_{op} \geq 16 \sqrt{n}) \leq 2^{-4n}.$
\end{lemma}
\begin{proof}
First, recall that $\mathbb{E}[M'] = 2\epsilon \cdot M$, so
$$M_{i,j}' - \mathbb{E}[M_{i,j}'] := 
\begin{cases}
      (1-2\epsilon)M_{i,j} & \text{w. pr. } \frac{1}{2} + \epsilon;\\
       -(1+2\epsilon)M_{i,j} & \text{w. pr. } \frac{1}{2} - \epsilon.
    \end{cases}
$$
Thus $\frac{1}{1+2\epsilon}(M'-\mathbb{E}[M'])$ has all the elements bounded by $1$ in absolute value. By using the exact same argument of Lemma~\ref{preadv-second-ineq}, we can show that $\Pr(\|M'-\mathbb{E}[M']\|_{op} \geq 16 \sqrt{n}) \leq 2^{-4n}$. Now, by Lemma~\ref{inftone-vs-op}, it holds $\|M'-\mathbb{E}[M']\|_{op} \geq \frac{1}{n} \cdot \|M'-\mathbb{E}[M']\|_{\inftone}$, so $$\Pr(\|M'-\mathbb{E}[M']\|_{\inftone} \geq 16n \sqrt{n}) \leq \Pr(\|M'-\mathbb{E}[M']\|_{op} \geq 16 \sqrt{n}) \leq 2^{-4n}.$$
\end{proof}

\begin{lemma}\label{postadv-second-ineq}
$\|M''-M'\|_{\inftone} \leq 2B;\ \|M''-M'\|_{op} \leq 2\sqrt{B}.$
\end{lemma}
\begin{proof}
Define $E:=M''-M'$. By definition, $E$ has $B$ non-zero entries, each of which is either $-2$ or $2$. Therefore, since each one of those entries can contribute by at most $2$ to the norm of $E$, $\|E\|_{\inftone} \leq 2B$. Moreover, by the same reason, $\|E\|_{F} \leq 2\sqrt{B}$. So, by Lemma~\ref{norms-ineq}, also $\|E\|_{op} \leq 2\sqrt{B}$.
\end{proof}

By putting those lemmas together, we can relate the final matrix $M''$ to the initial matrix $M$.

\begin{theorem}\label{postadv-displ}
With probability at least $1 -2^{-4n}=1-o(1)$,
$$\|M''-2\epsilon \cdot M\|_{\inftone} \leq 16n \sqrt{n} + 2B;\ \|M''-2\epsilon \cdot M\|_{op} \leq 16 \sqrt{n} + 2\sqrt{B}$$
\end{theorem}
\begin{proof}
By the triangle inequality, $\|M''-2\epsilon \cdot M\|_{\inftone} \leq \|M''-M'\|_{\inftone} + \|M'-2\epsilon \cdot M\|_{\inftone}$. First, by Lemma~\ref{postadv-second-ineq}, it holds $\|M''-M'\|_{\inftone} \leq 2B$. Second, we have that $\mathbb{E}[M'] = 2\epsilon \cdot M$, so $\|M'-2\epsilon \cdot M\|_{\inftone} = \|M'-\mathbb{E}[M']\|_{\inftone}$. Now, by Lemma~\ref{postadv-first-ineq}, with high probability $\geq 1 -2^{-4n}=1-o(1)$, it holds $\|M'-\mathbb{E}[M']\|_{\inftone} \leq 16 n\sqrt{n}$. By putting everything together, we finally get that $\|M''-2\epsilon \cdot M\|_{\inftone} \leq 16 n\sqrt{n} + 2B$. The same exact strategy can be used to prove the bound for the operator norm too.
\end{proof}

\subsubsection{Sub-optimal Robustness of the Spectral Approach}
Let 
\begin{equation}\label{postadv-spectral-params}
    \epsilon = \omega(n^{-1/2}) \; \; \;  \mbox{and} \; \; \; B=o(\epsilon^2 n^2).
\end{equation}
Let us show that, for these parameters, the spectral approach is robust w.r.t. a post-adversary. By Theorem~\ref{postadv-displ}, with probability at least $1 - 2^{-4n}=1-o(1)$, it holds $\|M''-2\epsilon \cdot M\|_{op} \leq 16 \sqrt{n} + 2\sqrt{B} = o(\epsilon n)$. Therefore, we are back to the same exact setting we analyzed with the pre-adversary: we have a matrix $M''$ such that, with high probability, $\|M''-2\epsilon \cdot M\|_{op} \leq o(\epsilon n)$, as in Theorem~\ref{preadv-displ}.
Thus, as showed in Lemma~\ref{spectral-preadv-2}, the eigenvector of the leading eigenvector of $M''$ is within euclidean distance $o(1)$ from the main eigenvector of the original matrix $M$, implying that it can be effectively used to approximately reconstruct the clusters. Therefore, we can rely on Algorithm~\ref{alg:preadv-2}.

As we show in Section~\ref{sec:slimits}, as far as $B$ is concerned this analysis is nearly tight asymptotically for a wide range of values of $\epsilon$. Indeed, when $\epsilon = \Omega((\log(n)/n)^{1/3})$, by modifying  $B=\Theta(\epsilon^2 n^2)$ entries, the post-adversary can induce with high-probability a principal eigenvector that gives no information on the latent clustering. This makes the spectral algorithms like Algorithm~\ref{alg:preadv-2} fail and creates a gap between the information-theoretic threshold, which is $B=o(\epsilon n^2)$ (see Section~\ref{sec:infotheo}), and the reach of spectral methods. We believe that the same techniques can be used to prove that the same impossibility result holds for any $\epsilon = \omega(n^{-1/2})$, but we have not been able to prove it in this work.

In the following subsection we show that the gap can be eliminated thanks to an SDP-based algorithm.

\subsubsection{SDP to the rescue}
In this section we show that SDP can recover the cluster almost perfectly and with high probability all the way to the information-theoretic threshold against the post-adversary.
Let
\begin{equation}\label{postadv-params}
\epsilon = \omega(n^{-1/2}) \; \; \; \mbox{and} \; \; \; B=o(\epsilon n^2).
\end{equation}
Consider the following Semidefinite Program:
\begin{equation}\label{sdp-2}
\begin{array}{ll@{}ll}
\text{maximize}  & \displaystyle\sum_{i,j=1}^{n}{M_{ij}''\langle \bm{x}_i, \
\bm{y}_j \rangle} &\\
\text{subject to}& \|\bm{x}_i\|=1 , \bm{x}_i \in \mathbb{R}^n  & & i=1 ,\dots, n\\
&\|\bm{y}_i\|=1, \bm{y}_i \in \mathbb{R}^n   & & i=1 ,\dots, n
\end{array}
\end{equation}
Henceforth we shall refer to this program as \sdp.
By definition of SDP-norm, its maximum is $\|M''\|_{SDP}$. Given the optimal solution $\{\bm{x}_i^\ast\}_{i \in [n]},\{\bm{y}_i^\ast\}_{i \in [n]}$, consider the matrix $X$ where $X_{ij}:=\langle \bm{x}_i^\ast, \bm{y}_j^\ast \rangle \ \forall\ i,j \in [n]$. Then, $\|M''\|_{SDP} = M'' \bullet X$, where $\bullet$ is the Kronecker (element-wise) product. Since $M''$ is symmetric, $X$ is symmetric too. Solving \sdp\ is the key step in the reconstruction, carried out by Algorithm~\ref{alg:postadv-2}.
\begin{algorithm}
\caption{: input $M''$, $n$}
\label{alg:postadv-2}
\begin{algorithmic}[1]
\STATE $\mathcal{S}_1 \leftarrow \emptyset;\ \mathcal{S}_2 \leftarrow \emptyset$
\STATE Let $X $ be the solution matrix of $\sdp$ obtained through $\sdpsolve$
\STATE Let $\{\bm{u}^1, \dots,\bm{u}^n\}$  be an orthogonal basis of eigenvectors of $X$ with eigenvalues respectively $\{\lambda_i, i \in [n']\}$ obtained through \power
\STATE{Sample $\bm{u}^\ast\in \{\bm{u}^i, i \in [n]\}$ with probability distribution $\{\frac{\lambda_i}{n}, i \in [n]\}$}\label{uast-line}
\FOR{$i = 1,\dots,n$}
\IF{$\bm{u}^\ast_i > 0$}
\STATE $\mathcal{S}_1 \leftarrow \mathcal{S}_1 \cup \{i\}$
\ELSE
\STATE $\mathcal{S}_2 \leftarrow \mathcal{S}_2 \cup \{i\}$
\ENDIF
\ENDFOR
\STATE \textbf{Return } $\{\mathcal{S}_1,\mathcal{S}_2\}$
\end{algorithmic}
\end{algorithm}

The main difference between Algorithm~\ref{alg:postadv-2} and Algorithm~\ref{alg:preadv-2} is how the former computes the eigenvector of interest. First, Algorithm~\ref{alg:postadv-2} computes the matrix $X$ solution to \sdp. Second, it computes an orthogonal basis of eigenvectors for $X$ with the \power. Third, it samples an eigenvector of the basis according to an appropriate probability distribution. The use of $X$ is necessary because the main eigenvector of $M''$, as we have argued previously, could no longer be informative. Notice that $\{\nicefrac{\lambda_i}{n}, i \in [n]\}$ is a probability distribution since $\sum_{i=1}^{n}{\lambda_i} = \tr(X) = n$. We will show that, surprisingly, if we sample $\bm{u}^\ast\in \{\bm{u}^i, i \in [n]\}$ with probability distribution $\{\frac{\lambda_i}{n}, i \in [n]\}$, with high probability we get an eigenvector that is very close to a main eigenvector of the original matrix $M$, and we believe this sampling technique for the eigenvector $\bm{u}^\ast$ to be key to the functioning of our algorithm.

\begin{lemma}\label{postadv2-normbound}
With probability at least $1 - 2^{-4n}$,
$\|M''\|_{SDP} = M'' \bullet X \geq 2\epsilon  n^2 - 29n \sqrt{n} - 4B = 2\epsilon n^2 - o(\epsilon n^2).$
\end{lemma}
\begin{proof}
First, it holds $\|M\|_{\inftone} = n^2$. Consider the vector $\bm{x} = \bm{f}_1 - \bm{f}_2$, having $+1$ for elements in the first cluster and $-1$ for elements in the second cluster. This satisfies $\|\bm{x}\|_{\infty}=1$, so $n^2 \geq \|M\|_{\inftone} \geq |\bm{x}^TM\bm{x}| = n^2$. As a consequence, $\|2\epsilon \cdot M\|_{\inftone} = 2\epsilon n^2$. Since $\|M\|_{\inftone} \leq \|M\|_{SDP} \leq \sum_{i,j}{|M_{ij}|} = n^2$, we also have that $\|2\epsilon \cdot M\|_{SDP} = 2\epsilon n^2$. Second, by Lemma~\ref{postadv-displ}, with high probability $\geq 1 - 2^{-4n} = 1-o(1)$ it holds 
$$\|M''-2\epsilon \cdot M\|_{\inftone} \leq 16n \sqrt{n} + 2B = o(\epsilon n^2).$$
Third, by the triangle inequality,
$$M'' \bullet X = \|M''\|_{SDP} \geq \|2\epsilon \cdot M\|_{SDP} -  \|M''- 2\epsilon \cdot M\|_{SDP}.$$
Now, by Theorem~\ref{grothendieck} and by what we have just proved, $\|2\epsilon \cdot M\|_{SDP} = 2\epsilon n^2$ and $\|M''-2\epsilon \cdot M\|_{SDP} \leq 1.8 \cdot \|M''-2\epsilon \cdot M\|_{\inftone} \leq 1.8 \cdot (16n \sqrt{n} + 2B) \leq 29n \sqrt{n} + 4B$. Thus, by putting everything together, we finally get that
$$\|M''\|_{SDP} \geq 2\epsilon n^2 - 29n \sqrt{n} - 4B .$$
\end{proof}

\begin{corollary}\label{small-SDP-displ-2}
With probability at least $1 - 2^{-4n}$, 
$\|M''-2\epsilon \cdot M\|_{SDP} \leq 29n \sqrt{n} + 4B= o(\epsilon n^2).$
\end{corollary}

Since $X$ is symmetric, we can consider its spectral decomposition into orthogonal eigenvectors:
$$X = \sum_{i=1}^{n}{\lambda_i\bm{u}^i(\bm{u}^i)^T}.$$
Now, sample $\bm{u}^\ast$ among the eigenvectors $\{\bm{u}^i\}_{i \in [n]}$ of this basis, each with probability $\nicefrac{\lambda_i}{n}$. We claim that $\bm{u}^\ast$, with high probability, gives a very good clustering reconstruction, because it is very close to $\bm{v}$, the main eigenvector of $M$ (or to its opposite vector).

\begin{lemma}\label{sol-postadv2}
Let $\bm{u}^\ast$ be the eigenvector of the solution matrix $X$ of 
\sdp\ given by Algorithm~\ref{alg:postadv-2}, line~\ref{uast-line}. Then, with probability at least $1 - 2\sqrt{\nicefrac{29}{\epsilon \sqrt{n}} + \nicefrac{4B}{\epsilon n^2}} = 1-o(1)$, an eigenvector $\bm{v}$ of the leading eigenvalue of $M$ satisfies
$$\|\bm{u}^\ast - \bm{v}\|^2\leq 2\sqrt{\frac{29}{\epsilon \sqrt{n}} + \frac{4B}{\epsilon n^2}}=o(1).$$
\end{lemma}
\begin{proof}
First, we show that $M \bullet X \geq  n^2 - o( n^2)$. We have that $M \bullet X = \frac{1}{2\epsilon} \left( M'' \bullet X - (M''-2\epsilon \cdot M) \bullet X \right)$. Now, by Corollary~\ref{small-SDP-displ-2}, with high probability $\geq 1 - 2^{-4n} = 1-o(1)$, it holds $\|M''-2\epsilon \cdot M\|_{SDP} \leq 29n \sqrt{n} + 4B= o(\epsilon n^2)$, so $(M''-2\epsilon \cdot M) \bullet X \leq \|M''-2\epsilon \cdot M\|_{SDP} \leq 29n \sqrt{n} + 4B$, and by Lemma~\ref{postadv2-normbound} it holds $M'' \bullet X \geq 2\epsilon  n^2 - 29n \sqrt{n} - 4B$, implying that
$$M \bullet X \geq  n^2 - \frac{29n \sqrt{n}}{\epsilon} - \frac{4B}{\epsilon} = n^2 - o(n^2).$$
Now $X = \sum_{i=1}^{n}{\lambda_i\bm{u}^i(\bm{u}^i)^T}$ is positive semidefinite and $\sum_{i=1}^{n}{\lambda_i} = \tr(X) = \sum_{i=1}^{n}{\|\bm{x}_i\|^2} = n$. Therefore, $\{\lambda_i/n\}_i$ can be seen as a probability distribution. By definition of $X$, we can consider an orthogonal basis of eigenvectors for it, $\{\bm{u}^i\}_{i \in [n]}$, with corresponding eigenvalues $\{\lambda_i\}_{i \in [n]}$. It holds 
$$M \bullet X = n\sum_{i=1}^{n}{\frac{\lambda_i}{n}(\bm{u}^i)^TM\bm{u}^i}.$$
We can write $M=n\bm{v}\bm{v}^T$, where $\bm{v} = \frac{1}{\sqrt{n}}(\bm{f}_1 - \bm{f}_2)$ is its main unitary eigenvector, so that $(\bm{u}^i)^TM\bm{u}^i = n\langle \bm{u}^i, \bm{v}\rangle^2$. We get that, with high probability $\geq 1 - 2^{1-4n} = 1-o(1)$, it holds
$$\sum_{i=1}^{n}{\frac{\lambda_i}{n}\langle \bm{u}^i, \bm{v}\rangle^2} \geq 1 - \frac{29}{\epsilon \sqrt{n}} - \frac{4B}{\epsilon n^2} = 1 - o(1).$$
We can notice that the LHS is exactly equal to $\mathbb{E}[\langle \bm{u}^*, \bm{v}\rangle^2]$. Since $\langle \bm{u}^*, \bm{v}\rangle^2 \leq \|\bm{v}\|^2 = 1$, we can define the positive random variable $\chi:=1-\langle \bm{u}^*, \bm{v}\rangle^2$. We have that $\chi \geq 0$ and $\mathbb{E}[\chi] \leq \frac{29}{\epsilon \sqrt{n}} + \frac{4B}{\epsilon n^2} = o(1)$. Thus, by Theorem~\ref{markov}, we have that with high probability $\geq 1 - \sqrt{\frac{29}{\epsilon \sqrt{n}} + \frac{4B}{\epsilon n^2}}$, it holds
$\chi \leq \sqrt{\frac{29}{\epsilon \sqrt{n}} + \frac{4B}{\epsilon n^2}}$, implying that
$$|\langle \bm{u}^*, \bm{v}\rangle| \geq \langle \bm{u}^*, \bm{v}\rangle^2 \geq 1 - \sqrt{\frac{29}{\epsilon \sqrt{n}} + \frac{4B}{\epsilon n^2}} = 1 - o(1).$$
We can assume w.l.o.g. that $\langle \bm{u}^*, \bm{v}\rangle > 0$, because we just need to take the opposite of $\bm{v}$ to change the sign of $\langle \bm{u}^*, \bm{v}\rangle$. Therefore, conditioned on the previous events, it holds
$$\|\bm{v} -\bm{u}^\ast\|^2 = \langle \bm{v} -\bm{u}^\ast,\bm{v} -\bm{u}^\ast \rangle = 2 - 2\langle \bm{v}, \bm{u}^\ast \rangle \leq 2\sqrt{\frac{29}{\epsilon \sqrt{n}} + \frac{4B}{\epsilon n^2}}.$$
All the events hold together with probability $\geq 1 - \sqrt{\frac{29}{\epsilon \sqrt{n}} + \frac{4B}{\epsilon n^2}} - 2^{1-4n} \geq 1 - 2\sqrt{\frac{29}{\epsilon \sqrt{n}} + \frac{4B}{\epsilon n^2}}$ for sufficiently large $n$.
\end{proof}

We are now in a very similar situation to the pre-adversarial case:  we can compute an eigenvector that, with high probability, is very close to the main eigenvector of the original matrix $M$ from which, as the next theorem shows, the latent clustering can be almost perfectly recovered.

\begin{theorem}\label{postadv-2-works}
With probability $1-o(1)$, Algorithm~\ref{alg:postadv-2} correctly classifies $n-o(n)$ vertices, where the number of misclassified vertices is $ \leq 2\sqrt{\nicefrac{29n\sqrt{n}}{\epsilon} + \nicefrac{4B}{\epsilon}} = o(n)$.
\end{theorem}
\begin{proof}
By Lemma~\ref{sol-postadv2} $\bm{u}^\ast$, obtained in Algorithm~\ref{alg:postadv-2}, line~\ref{uast-line}, with high probability $1-o(1)$ satisfies $\|\bm{v} -\bm{u}^\ast\|^2 \leq 2\sqrt{\frac{29}{\epsilon \sqrt{n}} + \frac{4B}{\epsilon n^2}} = o(1)$, where $\bm{v}$ is a main eigenvector of the original matrix $M$. Now, unless we swap the clusters, we can write w.l.o.g. $\bm{v} = \frac{1}{\sqrt{n}}\bm{f}_1 - \frac{1}{\sqrt{n}}\bm{f}_2$, where $\bm{f}_i$ is the indicator vector of the $i^{th}$ cluster. Now, let $\mathcal{S}_{bad}:=\{i \in [n]: \bm{v}_i\bm{u}^\ast_i < 0\}$, i.e. the set of coordinates with swapped signs between $\bm{v}$ and $\bm{u}^\ast$. Those correspond exactly the misplaced vertices in Algorithm~\ref{alg:postadv-2}. However, if $i \in \mathcal{S}_{bad}$, since $|\bm{v}_i| \geq \frac{1}{\sqrt{n}}\ \forall\ i \in [n]$, it holds $|\bm{v}_i-\bm{u}^\ast_i| \geq \frac{1}{\sqrt{n}}$. Thus,
$$2\sqrt{\frac{29}{\epsilon \sqrt{n}} + \frac{4B}{\epsilon n^2}} \geq \|\bm{v} - \bm{u}^\ast\|^2 \geq \sum_{i \in \mathcal{S}_{bad}}{|\bm{v}_i-\bm{u}^\ast_i|^2} \geq \frac{|\mathcal{S}_{bad}|}{n},$$
implying that $|\mathcal{S}_{bad}| \leq n \cdot 2\sqrt{\nicefrac{29}{\epsilon \sqrt{n}} + \nicefrac{4B}{\epsilon n^2}} =  2\sqrt{\nicefrac{29n\sqrt{n}}{\epsilon} + \nicefrac{4B}{\epsilon}} = o(n)$.
\end{proof}

Let us analyse the running time of Algorithm~\ref{alg:postadv-2}.
Solving \sdp\ through \sdpsolve\ up to negligible error takes polynomial time. Likewise, computing an orthogonal basis of eigenvectors for $X$ up to negligible error takes polynomial time. Finally, the random sampling of $\bm{u}^*$ according to a discrete distribution with support size $n$ can also be done in time polynomial in $n$ \citep{bringmann2012efficient}. The resulting running time is thus polynomial.

==> algo-kgen-old.tex <==
\section{Reconstruction for an Arbitrary, but  Constant, Number of Clusters}\label{sec:largek}
Here we generalize the approach of Section~\ref{sec:k2} to the case in which there are $k=O(1)$ equinumerous clusters, each of size $\nicefrac{n}{k}$.

\subsection{Properties of the Input Matrices}
Notice that $M$ has rank $k$ now, for $k>2$, because it has $k$ distinct rows.
Recall the definition of $\bm{f}_i$, the characteristic vector of the $i$\textsuperscript{th} cluster: there are $1$'s in the positions corresponding to the elements of the cluster, and $0$ everywhere else.  
The rows of $M$ are spanned by the vectors $\{\bm{f}_i\}_{1 \leq i \leq k}$ and are linearly independent, as it can be shown by induction using the Gaussian elimination. Let us now look at the spectrum of $M$.

First, $0$ is an eigenvalue for $M$ whose eigenspace, for $k>2$, has dimension $n-k$ by the Dimension Theorem for vector spaces (it is described by a homogeneous equation whose associated matrix, $M$, has rank $k$). Second, $2 \cdot \nicefrac{n}{k}$ is also an eigenvalue whose eigenspace has dimension $k-1$. A  basis for it is $\{\bm{f}_i - \bm{f}_{i+1},\ 1 \leq i \leq n-1\}$. If $k>2$, we also have another eigenvalue: $-\nicefrac{(k-2)}{k} \cdot n = \big(\nicefrac{2}{k} - 1 \big) n$, whose eigenspace has dimension $1$ and is spanned by the eigenvector with all identical coordinates. There are no more eigenvectors, since the vector space $\mathbb{R}^{n}$ is the direct sum of these eigenspaces.

For our approach to work, we need a positive semidefinite matrix describing the clustering. Moreover, we would like the vector with all identical coordinates not to be an eigenvector with a high eigenvalue of this matrix. This is the reason why we introduce a suitable positive-semidefinite version of the input matrix.

\subsubsection{A Positive Semidefinite ``Correlation Matrix''}
We have seen that the original matrix $M$ has a negative eigenvalue $-\nicefrac{k-2}{k} \cdot n$ for $k > 2$, with corresponding unitary eigenvector $\bm{z}$ whose coordinates are all equal to $\nicefrac{1}{\sqrt{n}}$. This does not carry any information about the clusters. By removing it from the spectral decomposition, we can consider a different ``correlation matrix'',
$$
P := \frac{k}{2(k-1)} \cdot \left( M  + n\left(1 - \frac{2}{k}\right) \bm{z}\bm{z}^T \right), 
$$
whose entries are:
$$P_{i,j} := 
\begin{cases}
      1  & \text{if } i,j \text{ are in the same cluster;}\\
      - \frac{1}{k-1}        & \text{otherwise.}
    \end{cases}
$$
This matrix has rank $k-1$ and $k$ distinct rows, the last of which is the opposite of the sum of the previous $k-1$ ones. Its spectrum consists of:
\begin{itemize}
    \item the positive eigenvalue $\nicefrac{n}{k-1}$, whose eigenspace has dimension $k-1$, with a basis given by $\{\bm{f}_i-\bm{f}_{i+1}\}_{i \in [k-1]}$. Notice that this is also the subspace of vectors having all the same coordinates for vertices in the same cluster and having sum of coordinates equal to $0$;
    \item $0$, whose eigenspace has dimension $n-k+1$ and is the complementary to the previous eigenspace. This subspace is described by the equation $P\bm{x}=\bm{0}$.
\end{itemize}

It is useful to find an orthogonal basis for the eigenspace of $\nicefrac{n}{k-1}$. With the Grahm-Schmidt orthogonalization procedure, we can get an orthogonal basis $\bm{v}_1, \dots, \bm{v}_{k-1}$ where: 
\begin{equation}\label{orthbasis-P}
    \bm{v}_i:= \frac{1}{\sqrt{n/k}} \left( \frac{1}{\sqrt{i^2 + i}}\sum_{j=1}^{i}{\bm{f}_j} - \frac{i}{\sqrt{i^2 + i}}\bm{f}_{i+1} \right)\ \ \forall\ i \in [k-1].
\end{equation}
Equation~\ref{orthbasis-P} can be shown by induction. These vectors are mutually orthogonal, have identical coordinates for vertices in the same cluster and their coordinates sum to $0$. For instance, for $n=k=3$, we get,
$$\bm{v}_1 = \frac{1}{\sqrt{2}}(\bm{f}_1 - \bm{f}_2);\ \bm{v}_2 = \frac{1}{\sqrt{6}}(\bm{f}_1 + \bm{f}_2) - \frac{2}{\sqrt{6}}\bm{f}_3.$$
Notice that, for any $k$, any vector of the orthogonal basis detects at least one cluster. Moreover, any orthogonal vector in this subspace detects a bisection into disjoint clusters. We exploit this to reconstruct the original clusters iteratively.

\begin{lemma}\label{eigenspace-separating}
Let $\bm{v}_i$ be as in Equation~\ref{orthbasis-P}, for $i \in [k-1]$. And let $\bm{x}:=\sum_{i=1}^{k-1}{\lambda_i\bm{v}_i}$, where $\|x\| = \sum_{i=1}^{k-1}{\lambda_i^2 = 1}$. Then, there exists $i \neq j \in [k]$ such that, if $x^i$ is the coordinate of $\bm{x}$ along the vertices of the $i^{\text{th}}$ cluster, then
$$ |x^i - x^j| > \frac{1}{k \cdot \sqrt{n}}.$$
\end{lemma}
\begin{proof}
Let $y^i:=\sqrt{\frac{n}{k}}\cdot x^i$ for each $i \in [k]$. Assume by contradiction that our statement is false, so $|y^i-y^j| \leq \frac{1}{k^{3/2}}$ for each $i \neq j \in [k]$. First, we prove by induction that this implies $$ \frac{|\lambda_h|}{\sqrt{h^2+h}}  \leq \left( 1 - 2^{-h} \right) \frac{1}{k^{3/2}} \ \ \forall\ h \in [k-1].$$
\textbf{Base Case:} $h=1$. By our assumption, we have that $|y^1 - y^2| \leq \frac{1}{k^{3/2}}$. However, $|y^1 - y^2| = 2\frac{|\lambda_1|}{\sqrt{2}}$, thus $\frac{|\lambda_1|}{\sqrt{2}} \leq \frac{1}{2k^{3/2}} = (1 - 2^{-1})\frac{1}{k^{3/2}}$.\\
\textbf{Inductive Step:} $(h-1) \to h$. By our assumption, we have that $|y^h - y^{h+1}| \leq \frac{1}{k^{3/2}}$. However, $|y^h - y^{h+1}| = \big| 2\frac{\lambda_h}{\sqrt{h^2+h}} - \frac{\lambda_{h-1}}{\sqrt{h(h-1)}} \big| \geq 2\frac{|\lambda_h|}{\sqrt{h^2+h}} - \frac{|\lambda_{h-1}|}{\sqrt{h(h-1)}}$ by the triangle inequality. Moreover, by the inductive hypothesis, $\frac{|\lambda_{h-1}|}{\sqrt{h(h-1)}} \leq (1 - 2^{-(h-1)})\frac{1}{k^{3/2}}$. Thus, $\frac{|\lambda_h|}{\sqrt{h^2+h}}  \leq \left( 1 - 2^{-h} \right) \frac{1}{k^{3/2}}$.\\
As a consequence, we also get that $$|\lambda_h|  \leq \frac{\sqrt{h^2+h}}{k^{3/2}}\ \ \forall\ h \in [k-1].$$
However, by hypothesis, $\sum_{h=1}^{k-1}{|\lambda_h|^2} =1$. Therefore,
$$1 = \sum_{h=1}^{k-1}{|\lambda_h|^2} \leq \frac{1}{k^3} \sum_{h=1}^{k-1}{(h^2+h)} \leq \frac{1}{k^3} \sum_{h=1}^{k-1}{k(k-1)} \leq \frac{(k-1)^2k}{k^3} <  1,$$
which is a contradiction.
\end{proof}

It is also useful to find the value of some norms for the matrix $P$.

\begin{lemma}\label{P-norms}
We have that
$\|P\|_{F} = \nicefrac{n}{\sqrt{k-1}}$, $\|P\|_{op} = \nicefrac{n}{k-1}$, and $\|P\|_{SDP} = \nicefrac{n^2}{k-1}$. Moreover, when $k$ is even $\|P\|_{\infty \to 1} = \nicefrac{n^2}{k-1}$, while
when $k$ is odd,
$\|P\|_{\infty \to 1} = {n^2}(k+1 )/{k^2}$. 
\end{lemma}
\begin{proof}
The first two equations follow by what we have just said on the spectrum of $P$. As for the third one, it is easy to observe that the $\pm 1$ values in the corresponding norm should be symmetric. Let $\alpha$ be the number of $+1$ and $\beta=k-\alpha$ be the number of $-1$ in the optimal solution for the case $n=k$ (when $k<n$, it just suffices to multiply everything by $\frac{n^2}{k^2}$). We have that
$$\|M\|_{\infty \to 1} = 1 \cdot k + \frac{1}{k-1} \cdot [\alpha \cdot (\beta - \alpha + 1) + \beta \cdot (\alpha - \beta + 1)] = k + \frac{\alpha + \beta - (\alpha - \beta)^2}{k-1} .$$
Now, since $\alpha+\beta=k$, we get $
k + 1 + \frac{1}{k-1} - \frac{(2\alpha-k)^2}{k-1}$, which is maximized when $\alpha$ is as close as possible to $k/2$, yielding different values for $k$ even/odd, respectively $k+1 + \frac{1}{k-1} = \frac{k^2}{k-1}$ and $k+1$. The SDP norm of $P$ is the maximum of its Frobenius scalar product with a set of positive semidefinite matrices which contains $P$ itself, so it is 
$$\|P\|_{SDP} = P \bullet P = k + \frac{k^2-k}{(k-1)^2} = k + 1 + \frac{1}{k-1} = \frac{k^2}{k-1}.$$
\end{proof}

We finally need to assess how $P$ changes after a random perturbation as the one described in the random model for the original matrix $M$. We define
$$P_{i,j}' := 
\begin{cases}
      M_{i,j}' & \text{if } M_{i,j}'>0;\\
      \frac{M_{i,j}'}{k-1} & \text{otherwise. }
    \end{cases}
$$
Equivalently, we can write
$$P_{i,j}' = 
\begin{cases}
      P_{i,j} & \text{w. pr. } \frac{1}{2} + \epsilon;\\
      -P_{i,j} + \big( 1 - \frac{1}{k-1} \big) & \text{w. pr. } \frac{1}{2} - \epsilon.
    \end{cases}
$$
We can see that this turns $1$ into $-\frac{1}{k-1}$ w. pr. $\frac{1}{2} - \epsilon$ and vice versa. Observe that:
\begin{equation}\label{P'-exp}
\mathbb{E}[P'] = \left( \frac{1}{2} - \epsilon \right) \left( 1 - \frac{1}{k-1} \right)\cdot \mathbb{1} + 2\epsilon \cdot P,
\end{equation}
where $\mathbb{1}$ is the $n \times n$ matrix with all entries equal to $1$. We can now define $Q':=P'-\left( \frac{1}{2} - \epsilon \right) \left( 1 - \frac{1}{k-1} \right)\cdot \mathbb{1}$. By what we have said, this gives
$\mathbb{E}[Q'] = 2\epsilon \cdot P$, so $Q'$ can be used as a random perturbation of the matrix $2\epsilon \cdot P$.

\subsection{Pre-Adversarial Model}
Here we generalize the approach used for $k=2$ clusters: instead of recovering an approximation of the main eigenvector of the original input matrix, we recover an approximation of a basis of the eigenspace of the $k$ leading eigenvalues of the modified matrix $P$. This will reveal completely the actual clustering. We recall that $\epsilon = \omega(n^{-1/2})$, and $B=o(n^2)$ (Eq.~\ref{preadv-params}).

Consider the modified positive semidefinite ``correlation matrix'' $P$, defined as
$$P = \frac{k}{2(k-1)} \cdot \left( M  + n\left(1 - \frac{2}{k}\right) \bm{z}\bm{z}^T \right).$$
Analogously, define $P'$ from the intermediate matrix $M'$, obtained after the adversarial modifications, and $P''$ from the final matrix $M''$, obtained after the random perturbation too. Finally,  define $$Q:=P'' - \left( \frac{1}{2} - \epsilon \right) \left( 1 - \frac{1}{k-1} \right)\cdot \mathbb{1}.$$
We will recover the $k-1$ orthogonal eigenvectors associated to the $k-1$ largest eigenvalues of the random matrix $Q$, and then show that their eigenspace is very close to the one of the main eigenvectors of $P$. Therefore, we will use those vectors to reconstruct the $k$ clusters.

First, we can extend Theorem~\ref{preadv-displ} to this setting. The following results can be proved analogously.

\begin{theorem}\label{preadv-displ-P}
With high probability $\geq 1 -2^{-4n}=1-o(1)$, it holds
$$\|Q-2\epsilon \cdot P\|_{op} \leq 16 \sqrt{n} + 4\epsilon \cdot \sqrt{B} = o(\epsilon n).$$
\end{theorem}
\begin{proof}
First, analogously to Lemma~\ref{preadv-first-ineq}, it holds $\|P'-P\|_{op} \leq 2\sqrt{B}$, because there are $\leq B$ deterministic changes from $P$ to $P'$, each of amount $1 + \nicefrac{1}{k} \leq 2$. Second, analogously to Lemma~\ref{preadv-second-ineq}, with high probability $\geq 1 -2^{-4n}=1-o(1)$, it holds $\|P''-\mathbb{E}[P'']\|_{op} \leq 16 \sqrt{n}$. However, 
$$\mathbb{E}[P''] = \left( \frac{1}{2} - \epsilon \right) \left( 1 - \frac{1}{k-1} \right)\cdot \mathbb{1} + 2\epsilon \cdot P'.$$
Moreover, by definition of $Q$, we finally get that $Q - 2\epsilon \cdot P' = P'' - \mathbb{E}[P'']$.
Third, by the triangle inequality, $\|Q-2\epsilon \cdot P\|_{op} \leq \|Q-2\epsilon \cdot P'\|_{op} + 2\epsilon \|P'-P\|_{op}$. By putting everything together, we finally get that $\|Q-2\epsilon \cdot P\|_{op} \leq 16 \sqrt{n} + 4\epsilon \cdot \sqrt{B}$. Finally, we notice that $16 \sqrt{n} + 4\epsilon \cdot \sqrt{B} = o(\epsilon n)$ by Eq.~\ref{preadv-params}.
\end{proof}

We can now proceed by showing that the eigenspace of the $k-1$ leading eigenvalues of $Q$ is very close to the one of $P$. 

\begin{lemma}\label{spectral-preadv-k}
Let $\bm{v}_1'',\dots, \bm{v}_{k-1}''$ be unitary eigenvectors of the largest $k-1$ eigenvalues of $Q$, and let $\bm{v}_1,\dots, \bm{v}_{k-1}$ be an orthogonal basis of the largest eigenvalue of $P$. Let $V \in \mathbb{R}^{n,k-1}$ with $\bm{v}_1,\dots, \bm{v}_{k-1}$ as columns, and $V'' \in \mathbb{R}^{n,k-1}$ with $\bm{v}_1'',\dots, \bm{v}_{k-1}''$ as columns. Then, with high probability $\geq 1-2^{-4n} = 1-o(1)$, it holds 
$$\|VV^T - V''(V'')^T\|_F \leq \frac{8k}{\epsilon \sqrt{n}} + \frac{2k\sqrt{B}}{n} = o(1).$$
\end{lemma}
\begin{proof}
By what previously observed, $2\epsilon \cdot P$ is diagonalizable with eigenvalues $\frac{2}{k-1} \cdot \epsilon n$ and $0$, with the first having an eigenspace of dimension $k-1$. Thus, by Theorem~\ref{davis-kahan}, for any orthogonal basis of eigenvectors $\bm{v}_1,\dots, \bm{v}_{k-1}$ of the largest eigenvalue of $P$, it holds
$$\|VV^T - V''(V'')^T\|_F \leq \frac{\|Q-2\epsilon \cdot P\|_{op}}{\frac{2}{k-1} \cdot \epsilon n}.$$ Now, by Theorem~\ref{preadv-displ-P}, with high probability $\geq 1 -2^{-4n}=1-o(1)$, it holds $\|Q-2\epsilon \cdot P\|_{op} \leq 16 \sqrt{n} + 4\epsilon \cdot \sqrt{B} = o(\epsilon n)$, so 
$$\|VV^T - V''(V'')^T\|_F \leq \frac{16 \sqrt{n} + 4\epsilon \cdot \sqrt{B}}{\frac{2}{k-1} \cdot \epsilon n} \leq \frac{8k}{\epsilon \sqrt{n}} + \frac{2k\sqrt{B}}{n} = o(1).$$
\end{proof}

Thanks to this result, we can generalize our spectral approach. By recovering the eigenvectors of the $k-1$ largest eigenvalues of $Q$, we get a very good approximation of a basis of the eigenspace of the leading eigenvector of $P$, which can be used to set the clusters apart. 

\begin{algorithm}
\caption{: input $Q$, $n$, $k$}
\label{alg:preadv-k}
\begin{algorithmic}[1]
\STATE $\mathcal{S} \leftarrow \emptyset$
\STATE $\mathcal{U} \leftarrow [n]$
\STATE{Let $\{\bm{v}_1'', \dots,\bm{v}_{k-1}''\}$  be the $k-1$ main eigenvectors of $Q$ obtained through \power}\label{power-preadv-k}
\STATE $\{\mathcal{S}_1, \dots, \mathcal{S}_n\} \leftarrow \getclust(\{\bm{v}_1'', \dots,\bm{v}_{k-1}''\})$
\FOR{$\ell = 1,\dots,k-1$}
\REPEAT
\STATE{
Sample $i \in \mathcal{U}$}\label{pivot-choice} U.A.R.\UNTIL{$|\mathcal{S}_i \cap \mathcal{U}| \geq \frac{n}{2k}$}\label{welldef-preadv-k}
\STATE $\mathcal{S} \leftarrow \mathcal{S} \cup \{\mathcal{S}_i\cap \mathcal{U}\}$
\STATE $\mathcal{U} \leftarrow \mathcal{U} \setminus \mathcal{S}_i$
\ENDFOR
\STATE $\mathcal{S} \leftarrow \mathcal{S} \cup \{\mathcal{U}\}$
\STATE \textbf{return} $\mathcal{S}$
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{\getclust}
\label{getclust}
\begin{algorithmic}[1]
\STATE \textbf{Procedure} \getclust$(\{\bm{v}_1'', \dots,\bm{v}_{k-1}''\})$
\FOR{$i = 1,\dots,n$}
\FOR{$j = 1,\dots,n$}
\STATE $\mathcal{S}_{ij} \leftarrow \emptyset$
\FOR{$h = 1,\dots,k-1$}
\IF{$|(\bm{v}_h'')_i - (\bm{v}_h'')_j| > \frac{1}{2\sqrt{2n}}$}
\STATE $\mathcal{S}_{ij} \leftarrow \mathcal{S}_{ij} \cup \{h\}$
\ENDIF
\ENDFOR
\ENDFOR
\STATE $\mathcal{S}_i\leftarrow \{j \in [n]:\mathcal{S}_{i,j}  = \emptyset\}$
\ENDFOR
\STATE \textbf{return} $\{\mathcal{S}_1, \dots, \mathcal{S}_n\}$
\end{algorithmic}
\end{algorithm}

In Algorithm~\ref{alg:postadv-k}, we first obtain the eigenvectors of the $k-1$ leading eigenvalues of $Q$. After that, we use those to retrieve the cluster each element belongs to in procedure \getclust (Algorithm~\ref{getclust}): for each $i \in [n]$, this procedure computes a tentative cluster $\mathcal{S}_i$ for it, which contains all the indices whose corresponding elements in every generated eigenvector are close to the $i^{th}$ element. We will show that most of these tentative clusters are correct, meaning that they approximately reconstruct the cluster the element belongs to. Therefore, we can sample $k-1$ distinct approximate clusters and build the $k^{th}$ cluster with the remaining elements. With high probability, this procedure returns $k$ almost correct clusters.

First, we can use the previous results to show that the eigenspace of the obtained eigenvectors of $Q$ is ``close'' to the one of the leading eigenvectors of $P$.

\begin{lemma}\label{close-eigenspaces-preadv-k}
Let $\bm{v}_1'',\dots, \bm{v}_{k-1}''$ be the unitary eigenvectors of the largest $k-1$ eigenvalues of $Q$, as returned in line~\ref{power-preadv-k} of Algorithm~\ref{alg:preadv-k}, and let $\bm{v}_1,\dots, \bm{v}_{k-1}$ be an orthogonal basis of the largest eigenvalue of $P$. Then, with high probability $\geq 1-2^{-4n}$, for each $\bm{v}_h, h \in [k-1]$, it holds
$$\sum_{\ell=1}^{k-1}{\langle \bm{v}_h, \bm{v}_\ell'' \rangle^2} \geq 1 - \frac{64k^2}{\epsilon^2 n} - \frac{4k^2B}{n^2} = 1 - o(1).$$
Analogously, for each $\bm{v}_m'', m \in [k-1]$, it holds
$$\sum_{h=1}^{k-1}{\langle \bm{v}_h, \bm{v}_m'' \rangle^2} \geq 1 - \frac{64k^2}{\epsilon^2 n} - \frac{4k^2B}{n^2} = 1 - o(1).$$
\end{lemma}
\begin{proof}
With high probability $\geq 1-2^{-4n} = 1-o(1)$, by Lemma~\ref{spectral-preadv-k}, it holds 
$$\|VV^T - V''(V'')^T\|_F \leq \frac{8k}{\epsilon \sqrt{n}} + \frac{2k\sqrt{B}}{n}.$$ 
Now, we can notice that
$$\|VV^T - V''(V'')^T\|_F^2 = \sum_{i,j=1}^{n}{\left( \sum_{h=1}^{k-1}{\left( (\bm{v}_h)_i(\bm{v}_h)_j - (\bm{v}_h'')_i(\bm{v}_h'')_j \right)} \right)^2}$$
$$ = 2 \left( k-1 - \sum_{h=1}^{k-1}{\sum_{\ell=1}^{k-1}{\langle \bm{v}_h, \bm{v}_\ell'' \rangle^2}} \right).$$
Now fix a generic $h \in [k-1]$. For each $h' \in [k-1] \setminus \{h\}$, it holds $\sum_{\ell=1}^{k-1}{\langle \bm{v}_{h'}, \bm{v}_\ell'' \rangle^2} \leq \|\bm{v}_{h'}\|^2 = 1$, because it is the sum of the projections of orthogonal vectors onto $\bm{v}_{h'}$. Therefore, $\|VV^T - V''(V'')^T\|_F^2 \geq 2 \left( 1 - \sum_{\ell=1}^{k-1}{\langle \bm{v}_h, \bm{v}_\ell'' \rangle^2}\right)$. Moreover, we have shown that with high probability $$\|VV^T - V''(V'')^T\|_F^2 \leq \left( \frac{8k}{\epsilon \sqrt{n}} + \frac{2k\sqrt{B}}{n} \right)^2 \leq \frac{128k^2}{\epsilon^2 n} + \frac{8k^2B}{n^2} = o(1)$$ by using $(a+b)^2 \leq 2(a^2 + b^2)\ \forall\ a,b \in \mathbb{R}$. Therefore, we have that
$$\sum_{\ell=1}^{k-1}{\langle \bm{v}_h, \bm{v}_\ell'' \rangle^2} \geq 1 - \frac{64k^2}{\epsilon^2 n} - \frac{4k^2B}{n^2} = 1 - o(1).$$ Since everything is symmetric, the symmetric version of this inequality follows analogously.
\end{proof}

\begin{theorem}\label{preadv-k-works}
With high probability $1-o(1)$, Algorithm~\ref{alg:preadv-k} is well-defined and misplaces at most $o(n)$ vertices, where the number of misplaced vertices is at most $\frac{2048k^4}{\epsilon^2} + \frac{128k^4B}{n} = o(n)$.
\end{theorem}
\begin{proof}
We show that, with high probability $1-o(1)$, the Algorithm~\ref{alg:preadv-k} is well-defined, so it always succeeds in finding $i \in \mathcal{U}$ satisfying the condition of line~\ref{welldef-preadv-k}, and that our solution is an approximate reconstruction of the original clusters, i.e. that there is a bijection $\varphi$ from the returned sets $\mathcal{S}_i$ to the original clusters such that $|\mathcal{S}_i \Delta \varphi(\mathcal{S}_i)| \leq o(1)$.

First, for each eigenvector $\bm{v}_\ell'',\ell \in [k-1]$, we can define $\Tilde{\bm{v}}_\ell:=\sum_{h=1}^{k-1}{\langle \bm{v}_h, \bm{v}_\ell'' \rangle}\bm{v}_h$, which is the projection of $\bm{v}_\ell''$ onto the eigenspace spanned by $\{\bm{v}_1,\dots,\bm{v}_{k-1}\}$. Now, for each cluster $C$, we can define $\lambda_{\ell,C}$ as the coordinate of the vertices belonging to cluster $C$ in vector $\Tilde{\bm{v}}_\ell$, which is well-defined by what said about the spectrum of the input matrix. We can also define $\mathcal{S}_{bad}^{\ell,C}:=\{i \in C:|(\bm{v}_\ell'')_i-\lambda_{\ell,C}| > \frac{1}{4\sqrt{2n}}\}$, which is the set of indices of $C$ which have been moved far from $\lambda_C$ in $\bm{v}_\ell''$. By Lemma~\ref{close-eigenspaces-preadv-k}, with high probability $\geq 1 - 2^{-4n}$ it holds 
$\|\bm{v}_\ell''-\Tilde{\bm{v}}_\ell\|^2 \leq \frac{64k^2}{\epsilon^2 n} + \frac{4k^2B}{n^2} = o(1)$, thus
$$\frac{64k^2}{\epsilon^2 n} + \frac{4k^2B}{n^2} \geq \|\bm{v}_\ell''-\Tilde{\bm{v}}_\ell\|^2 \geq \sum_{i \in \mathcal{S}_{bad}^{\ell,C}}{|(\bm{v}_\ell'')_i-\lambda_{\ell,C}|^2} > \frac{|\mathcal{S}_{bad}^{\ell,C}|}{32n},$$
which implies that $|\mathcal{S}_{bad}^{\ell,C}| \leq \frac{2048k^2}{\epsilon^2} + \frac{128k^2B}{n} = o(n)$. Therefore, for each cluster, all but $o(n)$ vertices have coordinates close to $\lambda_{\ell,C}$ in $\bm{v}_\ell''$.

Second, we show that, for each pair of different clusters $C_1,C_2$, there exists $\bm{v}_\ell'', \ell \in [k-1]$, such that $|\lambda_{\ell,C_1} - \lambda_{\ell,C_2}| > \frac{1}{\sqrt{2n}}$. Consider the orthogonal basis of the eigenspace of the main eigenvalue of $P$, as defined at the beginning of this section. By its definition, for each $\bm{v}_\ell'', \ell \in [k-1]$, it holds $|\lambda_{\ell,C_1} - \lambda_{\ell,C_2}| = |\langle \bm{v}_1, \bm{v}_\ell'' \rangle| \cdot \sqrt{\frac{2k}{n}}$, because the coordinates of clusters $C_1,C_2$ only differ in vector $\bm{v}_1$, and by an amount of $\sqrt{\frac{2k}{n}}$ (they are $+ \sqrt{\frac{k}{2n}}$ and $- \sqrt{\frac{k}{2n}}$). By Lemma~\ref{close-eigenspaces-preadv-k}, it holds $\sum_{\ell=1}^{k-1}{\langle \bm{v}_1, \bm{v}_\ell'' \rangle^2} \geq 1 - \frac{64k^2}{\epsilon^2 n} - \frac{4k^2B}{n^2} = 1 - o(1)$, so there exists $\bm{v}_\ell'', \ell \in [k-1]$, such that $\langle \bm{v}_1, \bm{v}_\ell'' \rangle^2 > \frac{1}{k}$, implying that $|\lambda_{\ell,C_1} - \lambda_{\ell,C_2}| = |\langle \bm{v}_1, \bm{v}_\ell'' \rangle| \cdot \sqrt{\frac{2k}{n}} > \sqrt{\frac{2}{n}} > \frac{1}{\sqrt{2n}}$.

Third, consider $\mathcal{S}_{bad}:=\bigcup_{\ell \in [k-1],C}{\mathcal{S}_{bad}^{\ell,C}}$. By the union bound and by what just proven,
$$|\mathcal{S}_{bad}| \leq k^2 \cdot \left( \frac{2048k^2}{\epsilon^2} + \frac{128k^2B}{n} \right) = \frac{2048k^4}{\epsilon^2} + \frac{128k^4B}{n} = o(n).$$
Moreover, for each $i \notin \mathcal{S}_{bad}$, we have that:
\begin{itemize}
    \item if $j \notin \mathcal{S}_{bad}$ belongs to the same cluster $C_1$ of $i$, then for each $\bm{v}_\ell'',\ell \in [k-1]$ it holds $|(\bm{v}_\ell'')_i - (\bm{v}_\ell'')_j| \leq |(\bm{v}_\ell'')_i - \lambda_{\ell,C_1}| + |\lambda_{\ell,C_1} - (\bm{v}_\ell'')_j| \leq \frac{1}{2\sqrt{2n}}$ by the triangle inequality;
    \item if $j \notin \mathcal{S}_{bad}$ belongs to a different cluster $C_2$ from $i$, then there exists $\bm{v}_\ell'',\ell \in [k-1]$, such that $|\lambda_{\ell,C_1} - \lambda_{\ell,C_2}| > \frac{1}{\sqrt{2n}}$, implying that $|(\bm{v}_\ell'')_i - (\bm{v}_\ell'')_j| \geq |\lambda_{\ell,C_1} - \lambda_{\ell,C_2}| - |\lambda_{\ell,C_1} -(\bm{v}_\ell'')_i| - |(\bm{v}_\ell'')_j - \lambda_{\ell,C_2}| > \frac{1}{2\sqrt{2n}}$ by the triangle inequality.
\end{itemize}
We have shown that $\frac{1}{2\sqrt{2n}}$ is an appropriate distance threshold to separate elements in different clusters that do not belong to $\mathcal{S}_{bad}$.

Finally, by summing up, since $|\mathcal{S}_{bad}|=o(n)$, at each time step with high probability $\geq 1-o(1)$ we select $i \notin \mathcal{S}_{bad}$ from line~\ref{pivot-choice}. In this case, $\mathcal{S}_i$ has $\frac{n}{k} + o(n)$ elements, which are the elements in its cluster plus/minus eventual elements of $\mathcal{S}_{bad}$. The elements of $\mathcal{S}_{bad}$ could be wrongly added to $\mathcal{S}_i$, or wrongly removed and associated to a different set of those. Since $k=O(1)$, with high probability $\geq 1-o(1)$ this happens for $k$ straight times. Under all these assumptions, only the elements in $\mathcal{S}_{bad}$ can be classified incorrectly, but they are at most $\frac{2048k^4}{\epsilon^2} + \frac{128k^4B}{n} = o(n)$ by Eq.~\ref{preadv-params}.
\end{proof}

\paragraph{Polynomial Running Time. } If we neglect the cost of the \power\ and of procedure \getclust, Algorithm~\ref{alg:preadv-k} has a linear cost in $n$. Exactly as shown for the case $k=2$, the running time of the \power is $poly(n)$ and it computes the eigenvectors with negligible error. It is also easy to observe that procedure \getclust\ has cost $O(n^2)$ because $k=O(1)$. Therefore, the total running time is still $poly(n)$.

\subsection{Post-Adversarial Model}
Here we generalize the approach used for $k=2$ clusters: instead of solving a single SDP and extracting a good eigenvector from the solution matrix, we do this process iteratively, because each eigenvector only partitions the set of vertices in two. The errors made during these bisections are under control and sum up to $o(n)$. We recall that $\epsilon = \omega(n^{-1/2})$, and $B=o(\epsilon n^2)$ (Eq.~\ref{postadv-params}).

\paragraph{Extending the SDP-Based Approach. } Here we use the positive semidefinite matrix $P$ instead of $M$, with its random perturbation $P'$ and its post-adversarial perturbation $P''$, which can be obtained from $M''$ by turning its negative entries to $-\frac{1}{k-1}$.  We also recall that 
$$\mathbb{E}[P'] = 2\epsilon \cdot P + \left( \frac{1}{2} - \epsilon \right) \left( 1 - \frac{1}{k-1} \right)\cdot \mathbb{1}.$$
We can define
$$Q=P'' - \left( \frac{1}{2} - \epsilon \right) \left( 1 - \frac{1}{k-1} \right)\cdot \mathbb{1}.$$
By doing so, $Q$ can be seen as a perturbation of $2\epsilon \cdot P$, which is a positive semidefinite matrix. Thus, it can be effetively used as input matrix for an SDP that aims to reconstruct the clusters.

\paragraph{The Need for Recursion. } Algorithm~\ref{alg:preadv-k} avoids recursion by obtaining an approximation of the entire basis of eigenvectors of the leading eigenvalue of the original matrix, and we wondered if we could do the same in the post-adversarial model. However, we believe recursion to be difficult to bypass. We defined $Q$ so that $Q \sim 2\epsilon \cdot P$. Then, in our SDP, we look for a positive semidefinite matrix $X$ maximizing $Q \bullet X$. Since $P \bullet X$ is maximized at $X = P$, by maximizing $Q \bullet X \sim 2\epsilon \cdot P \bullet X$ we hoped to recover a perturbated form of the matrix $P$, i.e. we hoped that $X \sim P$. However, we will see why this could not happen. Take $k$ even and consider a partition of the clusters into two groups with $\nicefrac{k}{2}$ clusters each. Let $B$ be the corresponding \emph{bisecting} matrix: it has $B_{ij}=1$ if and only if $i,j$ belong to clusters in the same group (half), $B_{ij}=-1$ otherwise. It is clear that the matrix $B$ only gives information about a bisection of the vertices, but it does not allow a complete clustering reconstruction, while $P$ does. We can notice that
$$P \bullet P = P \bullet B = \frac{n^2}{k-1}.$$
As a consequence, $P\bullet X$ is maximized both at $X=B$ and $X=P$. Therefore, $Q\bullet P$ could be maximized by a matrix $X \sim B$ as well as a matrix $X \sim P$. In other words, the matrix $X$ could only give information about a bisection, instead of allowing to reconstruct all of the clusters simultaneously. This is why, with our current method, we cannot hope to avoid a recurring procedure. We do not yet know if adding extra constraints to the SDP can rule out undesired solutions --- we believe this to be an interesting question for future work.

\subsubsection{General Properties}

Analogously to what has been done with $k=2$ clusters, we can prove the following norm inequalities.

\begin{lemma}\label{postadv-k-first-ineq}
$$\Pr(\|P'-\mathbb{E}[P']\|_{\inftone} \geq 16n \sqrt{n}) \leq 2^{-4n}.$$
\end{lemma}
\begin{proof}
First, it holds
$$P_{i,j}' - \mathbb{E}[P_{i,j}'] := 
\begin{cases}
      (1-2\epsilon)P_{i,j} - \left( \frac{1}{2} - \epsilon \right) \left( 1 - \frac{1}{k-1} \right) & \text{w. pr. } \frac{1}{2} + \epsilon;\\
       -(1+2\epsilon)P_{i,j} + \left( \frac{1}{2} + \epsilon \right) \left( 1 - \frac{1}{k-1} \right) & \text{w. pr. } \frac{1}{2} - \epsilon.
    \end{cases}
$$
Thus $\frac{1}{1+2\epsilon}(P'-\mathbb{E}[P'])$ has all the elements bounded by $1$ in absolute value. By using the exact same argument of Lemma~\ref{preadv-second-ineq}, we can show that $\Pr(\|P'-\mathbb{E}[P']\|_{op} \geq 16 \sqrt{n}) \leq 2^{-4n}$. Now, by Lemma~\ref{inftone-vs-op}, it holds $\|P'-\mathbb{E}[P']\|_{op} \geq \frac{1}{n} \cdot \|P'-\mathbb{E}[P']\|_{\inftone}$, so $$\Pr(\|P'-\mathbb{E}[P']\|_{\inftone} \geq 16n \sqrt{n}) \leq \Pr(\|P'-\mathbb{E}[P']\|_{op} \geq 16 \sqrt{n}) \leq 2^{-4n}.$$
\end{proof}

We can also bound the norm displacement after the post-adversary intervention.

\begin{lemma}\label{postadv-k-second-ineq}
$$\|P''-P'\|_{\inftone} \leq 2B = o(\epsilon n^2).$$
\end{lemma}
\begin{proof}
Let $P''=P'+E$, where $E$, the matrix of adversarial changes, has $B=o(\epsilon n^2)$ non-zero entries, all with absolute value $1+\nicefrac{1}{k-1} \leq 2$. Therefore, $\|E\|_{\inftone} \leq 2B$.
\end{proof}

Consider the auxiliary matrix $Q$, defined as:
$$ Q:= P'' - \left( \frac{1}{2} - \epsilon \right) \left( 1 - \frac{1}{k-1} \right)\cdot \mathbb{1}.$$

\begin{lemma}\label{small-norm-diff}
With high probability $\geq 1 - 2^{-4n} = 1-o(1)$, it holds
$$\|Q-2\epsilon \cdot P\|_{\inftone} \leq 16n\sqrt{n} + 2B = o(\epsilon n^2).$$
\end{lemma}
\begin{proof}
By definition of $Q$ and $P'$, we get that 
$$Q - 2\epsilon \cdot P = (P'' - P') + (P' - \mathbb{E}[P']).$$
By Lemma~\ref{postadv-k-first-ineq}, with probability $\geq 1 - 2^{-4n}$ it holds $\|P'-\mathbb{E}[P']\|_{\inftone} \leq 16n \sqrt{n}$; by Lemma~\ref{postadv-k-second-ineq}, it holds $\|P''-P'\|_{\inftone} \leq 2B$. By putting everything together and using the triangle inequality, we finally get that with high probability ($\geq 1 - 2^{-4n}$)
$$\|Q-2\epsilon \cdot P\|_{\inftone} \leq 16n\sqrt{n} + 2B = o(\epsilon n^2).$$
\end{proof}

\subsubsection{A Recursive SDP-Based Approach} 

Consider the following SDP:
\begin{equation}\label{sdp-postk}
\begin{array}{ll@{}ll}
\text{maximize}  & \displaystyle\sum_{j=1}^{n}{Q_{ij}\langle \bm{x}_i, \bm{y}_j \rangle} &\\
\text{subject to}& \|\bm{x}_i\|=1 , \bm{x}_i \in \mathbb{R}^n  & & i=1 ,\dots, n\\
&\|\bm{y}_i\|=1, \bm{y}_i \in \mathbb{R}^n   & & i=1 ,\dots, n
\end{array}
\end{equation}
The maximum of this SDP is equal to $\|Q\|_{SDP}$. Given the optimal solution $\{\bm{x}_i^\ast\}_{i \in [n]},\{\bm{y}_i^\ast\}_{i \in [n]}$, consider the matrix $X$ where $X_{ij}:=\langle \bm{x}_i^\ast, \bm{y}_j^\ast \rangle \ \forall\ i,j \in [n]$. Then, $\|Q\|_{SDP} = Q \bullet X$, where $\bullet$ represents the Kronecker (element-wise) product. Since $Q$ is symmetric, by a well-known characteristic of SDPs, $X$ is symmetric too. The following lemma holds.

\begin{lemma}\label{postadvk-normbound}
With high probability ($\geq 1 - 2^{-4n}$), it holds
$$\|Q\|_{SDP} = Q \bullet X \geq \frac{2}{k-1} \cdot \epsilon n^2 - 29n \sqrt{n} - 4B = \frac{2}{k-1} \cdot \epsilon n^2 - o(\epsilon n^2).$$
\end{lemma}
\begin{proof}
By the triangle inequality, we have that
$$\|Q\|_{SDP} \geq 2\epsilon \cdot \|P\|_{SDP} - \|Q-2\epsilon \cdot P\|_{SDP}.$$
Now, by Lemma~\ref{small-norm-diff}, with high probability $\geq 1 - 2^{-4n} = 1-o(1)$, it holds
$\|Q-2\epsilon \cdot P\|_{\inftone} \leq 16n\sqrt{n} + 2B = o(\epsilon n^2)$ so, by Theorem~\ref{grothendieck}, we get that 
$$\|Q-2\epsilon \cdot P\|_{SDP} \leq 1.8 \cdot (16n\sqrt{n} + 2B) \leq 29n\sqrt{n} + 4B  =o(\epsilon n^2).$$
Moreover, by Lemma~\ref{P-norms}, we get that 
$\|P\|_{SDP} = \frac{n^2}{k-1}$.
By substituting these above, and exploiting Eq.~\ref{postadv-params}, we finally get that
$$\|Q\|_{SDP} \geq  \frac{2}{k-1} \cdot \epsilon n^2 - 29n \sqrt{n} - 4B = \frac{2}{k-1} \cdot \epsilon n^2 - o(\epsilon n^2) .$$
\end{proof}

Since $X$ is symmetric, we can consider its spectral decomposition into orthogonal eigenvectors:
$$X = \sum_{i=1}^{n}{\lambda_i\bm{u}^i(\bm{u}^i)^T}.$$

Now, consider $\bm{u}^\ast$ picked randomly in $\{\bm{u}^i, i \in [n]\}$, where $\bm{u}^i$ is picked with probability proportional to $\lambda_i$. We will show that, with high probability, $\bm{u}^\ast$ gives a separation of the vertices into two sets, each containing at least one original cluster, and putting almost always together vertices belonging to the same cluster. This random sampling technique for an eigenvector is the same used for $k=2$ clusters.

\begin{lemma}\label{sol-postadvk}
Consider $Q \in \mathbb{R}^{n,n}$ such that $\|Q - 2\epsilon \cdot P\|_{\inftone} \leq f(n,B,\epsilon) =  o(\epsilon n^2)$. Let $X$ be the (symmetric positive semidefinite) solution matrix of SDP~\ref{sdp-postk} w.r.t. $Q$, let $\{\bm{u}^i\}_{i \in [n]}$ an orthogonal basis of eigenvectors for $X$ with eigenvalues respectively $\{\lambda_i\}_{i \in [n]}$. Pick $\bm{u}^* \in \{\bm{u}^i\}_{i \in [n]}$ randomly, where each $\bm{u}^i$ is chosen with probability $\frac{\lambda_i}{n}$. Then, with high probability $\geq 1- 2k \cdot \sqrt{\frac{f(n,B,\epsilon)}{\epsilon n^2}} - 2^{-4n}= 1-o(1)$, there exists $\bm{v}$ eigenvector of $P$ with eigenvalue $\frac{n}{k-1}$ such that 
$$\|\bm{u}^\ast - \bm{v}\|^2 \leq 4k \cdot \sqrt{\frac{f(n,B,\epsilon)}{\epsilon n^2}} =o(1).$$
\end{lemma}
\begin{proof}
First, by definition of $X$ it holds 
$\|Q\|_{SDP} = Q \bullet X .$ Now, by the triangle inequality, $|\|Q\|_{SDP}-2\epsilon \cdot \|P\|_{SDP}| \leq \|Q - 2\epsilon \cdot P\|_{SDP}$. However, by Theorem~\ref{grothendieck}, $\|Q - 2\epsilon \cdot P\|_{SDP} \leq 1.8\cdot \|Q - 2\epsilon \cdot P\|_{\inftone} \leq 1.8 \cdot f(n,B,\epsilon) = o(\epsilon  n^2)$. Thus, by Lemma~\ref{P-norms}, we get that $\|Q \|_{SDP} \geq 2\epsilon\| P\|_{SDP} - \|Q - 2\epsilon\cdot P \|_{SDP} \geq \frac{2}{k-1} \cdot \epsilon n^2 - 1.8 \cdot f(n,B,\epsilon) = \frac{2}{k-1} \cdot \epsilon n^2 - o(\epsilon n^2)$.
Now, recall that $\|Q - 2\epsilon \cdot P\|_{SDP} \leq 1.8 \cdot f(n,B,\epsilon)$, so $|(Q - 2\epsilon \cdot P) \bullet X| \leq \|Q - 2\epsilon \cdot P\|_{SDP} \leq 1.8 \cdot f(n,B,\epsilon) = o(\epsilon n^2)$. So, by the triangle inequality, we also get that $ (2\epsilon P) \bullet X \geq Q \bullet X - |(Q - 2\epsilon \cdot P) \bullet X| \geq \|Q\|_{SDP} - \|Q - 2\epsilon \cdot P\|_{SDP}$, implying that $(2\epsilon P) \bullet X \geq \frac{2}{k-1} \cdot \epsilon n^2 - 3.6 \cdot f(n,B,\epsilon) = \frac{2}{k-1} \cdot \epsilon n^2 - o(\epsilon n^2)$, i.e. that
\begin{equation}\label{X-also-good-for-P}
P \bullet X \geq \frac{n^2}{k-1}  - \frac{1.8}{\epsilon} \cdot f(n,B,\epsilon) \geq \frac{n^2}{k-1}  - \frac{2}{\epsilon} \cdot f(n,B,\epsilon) = \frac{n^2}{k-1} - o( n^2).
\end{equation}
Now, we can use the spectral decomposition $X = \sum_{i=1}^{n}{\lambda_i\bm{u}^i(\bm{u}^i)^T}$ is positive semidefinite, and $\sum_{i=1}^{n}{\lambda_i} = \tr(X) = \sum_{i=1}^{n}{\|\bm{x}_i\|^2} = n$. Therefore, $\{\lambda_i/n\}_i$ can be seen as a probability distribution. So it holds 
$$P \bullet X = n\sum_{i=1}^{n}{\frac{\lambda_i}{n}(\bm{u}^i)^T P\bm{u}^i}.$$
However, $P = \frac{n}{k-1}\sum_{j=1}^{k-1}{\bm{v}_j\bm{v}_j^T}$ and it is positive semidefinite, so $|(\bm{u}^i)^T P \bm{u}^i| = \frac{n}{k-1}\sum_{j=1}^{k-1}{\langle \bm{v}_j, \bm{u}^i \rangle^2} $ for each vector $\bm{u}^i$, implying that
$$\sum_{i=1}^{n}{\frac{\lambda_i}{n}\sum_{j=1}^{k-1}{\langle \bm{v}_j, \bm{u}^i \rangle^2}} = \frac{k-1}{n^2} \cdot P \bullet X \geq 1 - \frac{2(k-1)}{\epsilon n^2} \cdot f(n,B,\epsilon) \geq 1 - \frac{2k}{\epsilon n^2} \cdot f(n,B,\epsilon).$$
We can notice that the LHS is exactly $\mathbb{E}\left[\sum_{j=1}^{k-1}{\langle \bm{v}_j, \bm{u}^* \rangle^2}\right]$. So, we have shown that
\begin{equation}\label{exp-uast-P}
\mathbb{E}\left[\sum_{j=1}^{k-1}{\langle \bm{v}_j, \bm{u}^* \rangle^2}\right] = \sum_{i=1}^{n}{\frac{\lambda_i}{n}\sum_{j=1}^{k-1}{\langle \bm{v}_j, \bm{u}^i \rangle^2}} \geq 1 - \frac{2k}{\epsilon n^2} \cdot f(n,B,\epsilon) = 1 - o(1).
\end{equation}
Moreover, for each vector $\bm{u}$, the quantity $\sum_{j=1}^{k-1}{\langle \bm{v}_j, \bm{u} \rangle^2}$ is the squared norm of its projection onto the eigenspace of the eigenvalue $\frac{n}{k-1}$ of $P$, so it is always a quantity in $[0,1]$. Therefore, we can define the positive random variable $\chi:=1-\sum_{j=1}^{k-1}{\langle \bm{v}_j, \bm{u}^* \rangle^2}$. We have that $\chi \geq 0$ and $\mathbb{E}[\chi] \leq \frac{2k}{\epsilon n^2} \cdot f(n,B,\epsilon) = o(1)$. Thus, by Theorem~\ref{markov}, we have that with high probability $\geq 1 - \sqrt{\frac{2k}{\epsilon n^2} \cdot f(n,B,\epsilon)} \geq 1 - 2k\sqrt{\frac{f(n,B,\epsilon)}{\epsilon n^2}}$, it holds
$\chi \leq \sqrt{\frac{2k}{\epsilon n^2} \cdot f(n,B,\epsilon)}$, implying that
$$\sum_{j=1}^{k-1}{\langle \bm{v}_j, \bm{u}^\ast \rangle^2} \geq 1 - \sqrt{\frac{2k}{\epsilon n^2} \cdot f(n,B,\epsilon)} = 1 - o(1).$$
Now, let $$\bm{v}':=\sum_{j=1}^{k-1}{\langle \bm{v}_j, \bm{u}^\ast \rangle \bm{v}_j};\ \bm{v}:= \frac{\bm{v}'}{\|\bm{v}'\|}$$ be the normalized projection of $\bm{u}^\ast$ onto the eigenspace of the eigenvalue $\frac{n}{k-1}$ of $P$. It holds (using that $\sqrt{1-x} \geq 1 - x\ \forall\ x \in [0,1]$)
$$\|\bm{v} -\bm{u}^\ast\|^2 = \langle \bm{v} -\bm{u}^\ast,\bm{v} -\bm{u}^\ast \rangle = 2 - 2\langle \bm{v} ,\bm{u}^\ast \rangle = 2 - \frac{2}{\|\bm{v}'\|}\langle \bm{v}' ,\bm{u}^\ast \rangle =2 - 2\|\bm{v}'\| \leq
$$ 
$$  2 - 2\sqrt{1 - \sqrt{\frac{4k}{\epsilon n^2}\cdot f(n, B, \epsilon)}} \leq 2\sqrt{\frac{2k}{\epsilon n^2}\cdot f(n, B, \epsilon)} \leq 4k \cdot \sqrt{\frac{f(n,B,\epsilon)}{\epsilon n^2}} = o(1).$$
\end{proof}

As a consequence of Lemma~\ref{sol-postadvk}, Lemma~\ref{small-norm-diff} and Lemma~\ref{eigenspace-separating}, we can use $\bm{u}^\ast$ to separate $[n]$ into two smaller sets with minimal separation of vertices in the same cluster and with at least one cluster on each side. We see how through Algorithm \recur$([n],k,f,1)$ where $f=f(n,B,\epsilon)= 16n\sqrt{n} + 2B = o(\epsilon n^2)$. Before that, we need a formal definition.

\begin{definition}\label{matrix-restr}
Let $P \in \mathbb{R}^{n,n}$ matrix and let $\mathcal{S}_1,\mathcal{S}_2 \subseteq [n]$. We define $P^{\mathcal{S}_1,\mathcal{S}_2} \in \mathbb{R}^{|\mathcal{S}_1|,|\mathcal{S}_2|}$ be the sub-matrix of $P$ restricted only to the rows in $\mathcal{S}_1$ and to the columns in $\mathcal{S}_2$.
\end{definition}

\begin{algorithm}
\caption{\recur$(\mathcal{S},k',f,\gamma)$: input $\mathcal{S}$ set of indices, $k'$ number of clusters in $\mathcal{S}$, $f=f(n,B,\epsilon)=o(\epsilon n^2)$ such that $\|Q^{\mathcal{S},\mathcal{S}}-2\epsilon \cdot P^{\mathcal{S},\mathcal{S}}\|_{\inftone} \leq f$ (after having their negative entries multiplied by $\gamma$), $\gamma$ rescaling factor for the negative entries of $Q$. Global variables $n$, $k$, $Q$.}
\label{alg:postadv-k}
\begin{algorithmic}[1]
\STATE $\delta \leftarrow 4k \cdot \sqrt{\frac{f}{\epsilon n^2}}$
\STATE $n' \leftarrow |\mathcal{S}|$
\IF{$n' = n/k$}
\RETURN $\{\mathcal{S}\}$
\ENDIF
\STATE{Let $Q_{k'}$ be the matrix obtained from $Q^{\mathcal{S},\mathcal{S}}$ by multiplying its negative coordinates by $\gamma$}\label{line:rescale}
\STATE Let $X $ be the solution matrix of  SDP~\ref{sdp-postk} for $Q_{k'}$ obtained through \sdpsolve
\STATE Let $\{\bm{u}^1, \dots,\bm{u}^n\}$  be an orthogonal basis of eigenvectors of $X$ with eigenvalues respectively $\{\lambda_i, i \in [n']\}$ obtained through \power
\STATE Sample $\bm{u}^\ast\in \{\bm{u}^i, i \in [n']\}$ with probability distribution $\{\frac{\lambda_i}{n'}, i \in [n']\}$
\STATE{$t \leftarrow \getthr(\bm{u}^\ast,n',\delta)$ is the separating threshold according to vector $\bm{u}^\ast$}\label{line:thr}
\STATE Let $\mathcal{S}_1:=\{i \in \mathcal{S} :\bm{u}^\ast_i < t\}$
\STATE{$k'':=\lfloor \frac{|\mathcal{S}_1|}{n/k} \rceil$ (closest integer function $\lfloor \cdot \rceil$)}\label{adjust}
\IF{$k'' \in \{0,k'\}$}\label{if-postadvk}
\STATE \textbf{abort} (the algorithm failed)
\ENDIF
\STATE{$\mathcal{S}' \leftarrow \{i \in [n']:\bm{u}_i^* \text{ is among the } k'' \cdot \frac{n}{k}\text{ smallest coordinates of }\bm{u}_i^*\text{ (ties broken arbitrarily)}\}$}\label{fixing-card}
\STATE $f' \leftarrow k \cdot f + 4k\delta^{1/3} \cdot \epsilon (n')^2= o(\epsilon n^2)$ 
\STATE $\gamma' \leftarrow \frac{k'-1}{k''-1}$ scaling factor for $\mathcal{S}'$ because it now contains $k''$ clusters instead of $k'$
\STATE $\gamma'' \leftarrow \frac{k'-1}{k'-k''-1}$ scaling factor for $\mathcal{S}\setminus \mathcal{S}'$ because it contains the remaining $k' - k''$ clusters
\STATE$\mathcal{C}_1 \leftarrow \recur(\mathcal{S}', k'',f',\gamma')$
\STATE $\mathcal{C}_2 \leftarrow \recur(\mathcal{S}\setminus \mathcal{S}', k'-k'',f',\gamma'')$
\RETURN $\mathcal{C}_1 \cup \mathcal{C}_2$
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{\getthr}
\label{getthreshold}
\begin{algorithmic}[1]
\STATE \textbf{Procedure} \getthr$(\bm{u}, n',\delta)$
\STATE Let $\pi$ be the ordering permutation of vector $\bm{u}$, i.e. the permutation on $[n']$ s.t. $\bm{u}_{\pi(i)} \leq \bm{u}_{\pi(j)}\ \forall\ 1 \leq i \leq j \leq n'$
\STATE $t_{\min} \leftarrow \bm{u}_{\pi(\lceil \delta^{1/3}\cdot n' \rceil)}$
\STATE $t_{\max} \leftarrow \bm{u}_{\pi(n'-\lceil \delta^{1/3}\cdot n' \rceil)}$
\STATE Pick $t \in [t_{\min},t_{\max}]$ Uniformly At Random as the separating threshold for vector $\bm{u}$
\STATE \textbf{return} $t$
\end{algorithmic}
\end{algorithm}

Each iterative step of Algorithm~\ref{alg:postadv-k} is similar to Algorithm~\ref{alg:postadv-2}, but there are some main differences. 

First, we need to sample an appropriate threshold value for the eigenvector to separate the vertices (line~\ref{line:thr}), because we are getting an approximate eigenvector of the eigenspace of the leading vector of $P$, but we do not know exactly which approximate eigenvector we are getting. This is done by procedure \getthr. The threshold could be at any point in between the maximum and the minimum value of an eigenvector of $P$. However, since we only get an approximate eigenvector, we need to consider more robust order statistics to establish the feasible range for thresholds.

Second, we need to fix the cardinality of the bisection (line~\ref{fixing-card}) because we want the size of each partition to be an integer multiple of $\nicefrac{n}{k}$. 

Third, we need to carry the information about the number of clusters in each partition: this will be used to scale the negative elements of the input matrix $Q'$ of SDP~\ref{sdp-postk} (line~\ref{line:rescale}), so that this input matrix is always positive semidefinite. 

We also need to carry an estimate $f'$ of the distance in norm $\ell_{\infty}$-to-$\ell_{1}$ between the scaled matrix $Q'$ and the scaled original matrix $2\epsilon \cdot P$, whose negative entries are scaled like the ones of $Q'$.

We show that Algorithm~\ref{alg:postadv-k}, with high probability, always splits the solution into two ``smaller'' solutions that we can solve recursively, i.e. that the bisection of the input set $\mathcal{S}$ satisfies the condition of line~\ref{if-postadvk}. Moreover, we also show that the produced solutions only mislabel $o(n)$ vertices at each step. Before that, we prove an auxiliary lemma.

\begin{lemma}\label{small-displ}
Let $\bm{u},\bm{v} \in \mathbb{R}^n$ s.t. $\|\bm{u}-\bm{v}\|^2 \leq \delta$. Suppose that the coordinates of $\bm{v}$ can be partitioned into $k$ groups $P_1, \dots, P_k$ of $\frac{n}{k}$ elements each, such that all the coordinates in the same group $P_i$ are equal. Then, for each group $P_i$, there cannot be $\geq \delta^{1/3} \cdot n$ elements $j \in P_i$ such that $|\bm{u}_j-\bm{v}_j| > \frac{\delta^{1/3}}{\sqrt{n}}.$ 
\end{lemma}
\begin{proof}
Assume there is $P_i'\subseteq P_i$ such that $|P_i'|\geq \delta^{1/3} \cdot n$ and $|\bm{u}_j-\bm{v}_j| > \frac{\delta^{1/3}}{\sqrt{n}}\ \forall\ j \in P_i'$. Then,
$$\delta \geq \|\bm{v}-\bm{u}\|^2 \geq \sum_{j \in P_i'}{(\bm{u}_j-\bm{v}_j)^2}>  (\delta^{1/3} \cdot n) \cdot \left( \frac{\delta^{1/3}}{\sqrt{n}} \right)^2 \geq \delta,$$
which is a contradiction.
\end{proof}

In other words, in $\bm{u}$, all but $\leq \delta^{1/3}\cdot n$ elements of a group are within a distance $\leq \frac{\delta^{1/3}}{\sqrt{n}}$ from their coordinate in $\bm{v}$. The previous lemma is used to show that almost all the coordinates of approximate eigenvectors of $P$ are very close to the coordinates of the actual eigenvector of $P$. In order to get closer to the proof of the effectiveness of Algorithm~\ref{alg:postadv-k}, we state precise guarantees on what happens in the first round. To extend this to the recursive sub-problems, we need to make some adjustments to take into account the previous classification errors too.

\begin{lemma}\label{first-step-works}
Consider the invocation  of \recur$([n],k,f,1)$ where $f=f(n,B,\epsilon)= 16n\sqrt{n} + 2B = o(\epsilon n^2)$, and let $\delta:=4k \cdot \sqrt{\frac{f}{\epsilon n^2}} = 4k \cdot \sqrt{\frac{16}{\epsilon \sqrt{n}} + \frac{2B}{\epsilon n^2}} = o(1)$. With high probability $\geq 1 -2^{-4n} - 6k^2\cdot \delta^{1/3} = 1-o(1)$, the first sampled threshold $t$ does not satisfies the condition of line~\ref{if-postadvk} in Algorithm~\ref{alg:postadv-k}, so the algorithm does not fail. Moreover:
\begin{itemize}
    \item for each cluster, either $\mathcal{S}'$ or $\mathcal{S} \setminus \mathcal{S}'$ contains $\leq 2\delta^{1/3} \cdot n = o(n)$ of its vertices, meaning that there are $\leq 2k\delta^{1/3} \cdot n =  o(n)$ misplaced vertices overall in the first recursive step;
    \item let $\mathcal{A}$ be one of the sub-sets on which the algorithm is applied recursively (the same holds for the other subset), and let $\mathcal{A}^*$ be the union of the $k_{\mathcal{A}}$ clusters having $\geq \frac{n}{k} - 2\delta^{1/3} \cdot n$ elements in $\mathcal{A}$. Let $Q_{k_{\mathcal{A}}}$ be the matrix obtained from $Q$ by multiplying the negative entries by $\frac{k_{\mathcal{A}}-1}{k-1}$ and let $P_{k_{\mathcal{A}}}$ be the analogous matrix obtained from $P$. Then, 
    $$\|Q_{k_{\mathcal{A}}}^{\mathcal{A}^*,\mathcal{A}^*} - 2\epsilon \cdot P_{k_{\mathcal{A}}}^{\mathcal{A},\mathcal{A}}\|_{\inftone} \leq f' := k \cdot f(n,B,\epsilon) + 4k\delta^{1/3} \cdot \epsilon n^2= o(\epsilon n^2) .$$
\end{itemize}

\end{lemma}
\begin{proof}
By Lemma~\ref{small-norm-diff}, with high probability $\geq 1-2^{-4n}$ it holds $\|Q - 2\epsilon \cdot P\|_{\inftone} \leq f(n,B,\epsilon)= 16n\sqrt{n} + 2B = o(\epsilon n^2)$, and we consider this to be true from now on (by the union bound, the small probability of this to be false will sum up with the other encountered small probabilities). Therefore, by Lemma~\ref{minor-monotone}, for each set of indices $\mathcal{S} \subseteq [n]$, it also holds $\|Q^{\mathcal{S},\mathcal{S}} - 2\epsilon \cdot P^{\mathcal{S},\mathcal{S}}\|_{\inftone} \leq 16n\sqrt{n} + 2B = o(\epsilon n^2)$. 
Now, by Lemma~\ref{sol-postadvk}, with high probability $\geq 1 - \delta/2 = 1-o(1)$, there exists an eigenvector $\bm{v}$ of the leading eigenvalue $\frac{n}{k-1}$ of $P$ such that $\|\bm{v}-\bm{u}^\ast\|^2 \leq \delta = o(1)$. Now, let $v_{\max}:=\max_{i \in [n]}{\bm{v}_i}$ and $v_{\min}:=\min_{i \in [n]}{\bm{v}_i}$. By Lemma~\ref{eigenspace-separating}, it holds $|v_{\max} - v_{\min}| > \frac{1}{k\sqrt{n}}$. By Lemma~\ref{small-displ}, it follows that $|t_{\max} - v_{\max}| \leq \frac{\delta^{1/3}}{\sqrt{n}}$ and $|t_{\min} - v_{\min}| \leq \frac{\delta^{1/3}}{\sqrt{n}}$. As a consequence, we have that
$$\Pr\left( t \in \left[v_{\min}+\frac{\delta^{1/3}}{\sqrt{n}},v_{\max}-\frac{\delta^{1/3}}{\sqrt{n}}\right] \right) \geq  \frac{|v_{\max} - v_{\min}| - 2\frac{\delta^{1/3}}{\sqrt{n}}}{|v_{\max} - v_{\min}| + 2\frac{\delta^{1/3}}{\sqrt{n}}} \geq$$
$$1 - \frac{4\frac{\delta^{1/3}}{\sqrt{n}}}{\frac{1}{k\sqrt{n}}+2\frac{\delta^{1/3}}{\sqrt{n}}} \geq 1 - 4k \cdot \delta^{1/3} = 1-o(1).$$
However, if $t \in \left[v_{\min}+\frac{\delta^{1/3}}{\sqrt{n}},v_{\max}-\frac{\delta^{1/3}}{\sqrt{n}}\right]$, by Lemma~\ref{small-displ}, we separate almost exactly the clusters corresponding to the largest and the smallest coordinate of $\bm{v}$: $\geq \frac{n}{k} - \delta^{1/3} \cdot n$ elements of each cluster are split correctly according to the threshold, which makes the condition of line~\ref{if-postadvk} not satisfied and the algorithm does not fail. Now, we need to show that the bisection misplaces $o(n)$ vertices for each cluster. First, notice that, with high probability $\geq 1-\delta/2 = 1-o(1)$, by Lemma~\ref{small-displ}, for each cluster $C$ with coordinate $v_C$ in $\bm{v}$, all but $\delta^{1/3} \cdot n = o(n)$ elements of $C$ have coordinates of $\bm{u}^*$ in the interval $\left[v_C-\frac{\delta^{1/3}}{\sqrt{n}},v_C+\frac{\delta^{1/3}}{\sqrt{n}}\right]$. Therefore, by the union bound over all the clusters,
$$\Pr\left( \nexists\ C: t \in \left[v_C-\frac{\delta^{1/3}}{\sqrt{n}},v_C+\frac{\delta^{1/3}}{\sqrt{n}}\right] \right) \geq \frac{t_{\max}-t_{\min} - 2k \cdot \frac{\delta^{1/3}}{\sqrt{n}}}{t_{\max}-t_{\min}} \geq 1 - 2k^2\delta^{1/3}.$$
Thus, with probability $\geq 1 - 2k^2\delta^{1/3} = 1-o(1)$, we are outside each of those cluster intervals, meaning that, for each cluster, we can misplace $\leq \delta^{1/3} \cdot n$ vertices, for a total of $k\delta^{1/3} \cdot n$ total misplaced vertices according to the threshold bisection at $t$. Finally, the process of line~\ref{fixing-card}, can bring other $k\delta^{1/3} \cdot n$ mistakes (extra $\delta^{1/3} \cdot n$ for each clusters), for a total of $2k\delta^{1/3} \cdot n = o(n)$ misplaced vertices. By the union bound, everything holds with probability $\geq 1 -2^{-4n} - \nicefrac{\delta}{2} - 2k(k+2)\cdot \delta^{1/3} \geq 1 -2^{-4n} - 6k^2\cdot \delta^{1/3} $ (for sufficiently small $\delta$).

We now focus on the correctness of the estimate $f'$ of the $\ell_\infty$-to-$\ell_1$ norm of the generated subsets. First, we notice that $|\mathcal{A}| = |\mathcal{A}^*| = k_{\mathcal{A}} \cdot \frac{n}{k}$. Now, by what just proved, we can assume that $\mathcal{A} \Delta \mathcal{A}^* \leq 2k\delta^{1/3} \cdot n = o(n)$. By the triangle inequality 
$$\|2\epsilon \cdot P_{k_{\mathcal{A}}}^{\mathcal{A},\mathcal{A}} - Q_{k_{\mathcal{A}}}^{\mathcal{A}^*,\mathcal{A}^*}\|_{\inftone} \leq \|2\epsilon \cdot P_{k_{\mathcal{A}}}^{\mathcal{A},\mathcal{A}} - 2\epsilon \cdot P_{k_{\mathcal{A}}}^{\mathcal{A}^*,\mathcal{A}^*}\|_{\inftone}+ \|2\epsilon \cdot P_{k_{\mathcal{A}}}^{\mathcal{A}^*,\mathcal{A}^*} - Q_{k_{\mathcal{A}}}^{\mathcal{A}^*,\mathcal{A}^*}\|_{\inftone}.$$
By Lemma~\ref{small-norm-diff} we have that, under the previously mentioned events holding with high probability, $\|Q-2\epsilon \cdot P\|_{\inftone} \leq 16n\sqrt{n} + 2B = o(\epsilon n^2)$. Therefore, by Lemma~\ref{minor-monotone}, it follows that 
$$ \|2\epsilon \cdot P_{k_{\mathcal{A}}}^{\mathcal{A}^*,\mathcal{A}^*} - Q_{k_{\mathcal{A}}}^{\mathcal{A}^*,\mathcal{A}^*}\|_{\inftone} \leq \frac{k-1}{k_{\mathcal{A}}-1} \cdot \|2\epsilon \cdot P^{\mathcal{A}^*,\mathcal{A}^*} - Q^{\mathcal{A}^*,\mathcal{A}^*}\|_{\inftone}\leq  16k \cdot n\sqrt{n} + 2k \cdot B = o(\epsilon n^2).$$
Moreover, 
$$\|2\epsilon \cdot P_{k_{\mathcal{A}}}^{\mathcal{A},\mathcal{A}} - 2\epsilon \cdot P_{k_{\mathcal{A}}}^{\mathcal{A}^*,\mathcal{A}^*}\|_{\inftone} = 2 \epsilon \cdot \| P_{k_{\mathcal{A}}}^{\mathcal{A},\mathcal{A}} -  P_{k_{\mathcal{A}}}^{\mathcal{A}^*,\mathcal{A}^*}\|_{\inftone}.$$
Since $\mathcal{A} \Delta \mathcal{A}^* \leq 2k\delta^{1/3} \cdot n = o(n)$ and the entries of $P_{k_{\mathcal{A}}}$ are bounded in absolute value by $1$, we get that $\| P_{k_{\mathcal{A}}}^{\mathcal{A},\mathcal{A}} -  P_{k_{\mathcal{A}}}^{\mathcal{A}^*,\mathcal{A}^*}\|_{\inftone} \leq (2k\delta^{1/3} \cdot n) \cdot (2n) = 4k\delta^{1/3}n^2  = o(n^2)$. By putting everything together, we finally get that
$$\|Q_{k_{\mathcal{A}}}^{\mathcal{A}^*,\mathcal{A}^*} - 2\epsilon \cdot P_{k_{\mathcal{A}}}^{\mathcal{A},\mathcal{A}}\|_{\inftone} \leq k \cdot f + 4k\delta^{1/3}n^2 \leq 16k \cdot n\sqrt{n} + 2k \cdot B + 4k\delta^{1/3}n^2 \cdot \epsilon n^2= o(\epsilon n^2).$$
\end{proof}

We are now ready to extend the previous lemma to any recursive invocation of \recur.

\begin{theorem}\label{recur-works}
Consider a generic invocation  of \recur$(\mathcal{S},k',f,\gamma)$ originated from the first invocation of \recur$([n],k,16n\sqrt{n} + 2B,1)$, and let $\delta:=4k \cdot \sqrt{\frac{f}{\epsilon n^2}}$. With high probability $\geq 1-o(1)$:
\begin{itemize}
    \item for each cluster $C$, either $|C \cap \mathcal{S}| \leq o(n)$ or $|C \cap \mathcal{S}| \geq \frac{n}{k} - o(n)$, and there are exactly $k'$ clusters satisfying the second condition;
    \item let $\mathcal{S}^*$ be the union of the $k'$ clusters having $\geq \frac{n}{2k}$ elements in $\mathcal{S}$, let $Q_{k'}$ be the matrix obtained from $Q$ by multiplying the negative entries by $\gamma$, and let $P_{k'}$ be the analogous matrix obtained from $P$. Then, 
    $$\|Q_{k'}^{\mathcal{S},\mathcal{S}} - 2\epsilon \cdot P_{k'}^{\mathcal{S}^*,\mathcal{S}^*}\|_{\inftone} \leq f = o(\epsilon n^2) .$$
    \item if $k' > 1$, the first sampled threshold $t$ does not satisfies the condition of line~\ref{if-postadvk} in Algorithm~\ref{alg:postadv-k}, so the algorithm does not fail.
\end{itemize}
\end{theorem}
\begin{proof}
We show the Theorem by induction on the number of recursive calls each invocation of \recur\ comes from. 

\textbf{Base Case. } We start with the first invocation, i.e. \recur$([n],k,16n\sqrt{n} + 2B,1)$. First, each one of the $k$ clusters has $\frac{n}{k}$ elements in common with $[n]$. Second, by Lemma~\ref{small-norm-diff}, it holds $\|Q - 2\epsilon \cdot P\|_{\inftone} \leq  16n\sqrt{n} + 2B = o(\epsilon n^2)$, as desired. Finally, by Lemma~\ref{first-step-works}, with high probability $1 - o(1)$ the algorithm samples an appropriate threshold $t$ and it does not fail. Thus, everything holds in the first invocation of \recur.

\textbf{Inductive Step: from $(\mathcal{S},k',f,\gamma)$ to $(\mathcal{S}',k'',f',\gamma')$. } This follows the exact same steps of the proof of Lemma~\ref{first-step-works}, which can also be seen as a special case, proving the inductive step from the first invocation of \recur\ to its direct calls. We quickly go through these steps. Let $n':=|\mathcal{S}|$. We start from the fact that $Q_{k'}$, thanks to the scaling by $\gamma'$, becomes positive semidefinite. Moreover, let $\mathcal{S}^*$ be defined as in the statement of the lemma. By inductive hypothesis we get that, with high probability, $\|Q_{k'}^{\mathcal{S},\mathcal{S}} - 2\epsilon \cdot P_{k'}^{\mathcal{S}^*,\mathcal{S}^*}\|_{\inftone} \leq f = o(\epsilon n^2)$. This is the only necessary ingredient to show that, by Lemma~\ref{sol-postadvk}, with high probability  there exists $\bm{v}$ eigenvector of the leading eigenvalue of $P_{k'}$ such that 
$$\|\bm{u}^\ast - \bm{v}\|^2 \leq 4k' \cdot \sqrt{\frac{f}{\epsilon (n')^2}} =o(1).$$
We now notice that $P_{k'}$ is the positive semidefinite ``correlation matrix'' of a set of $k'$ clusters with size $\frac{n}{k}$. Apart from a normalization factor that depends on $k,k'$, it has the same eigenvectors and eigenvalues of the positive semidefinite ``correlation matrix'' $P'$ of a set of $k'$ clusters with size $\frac{n}{k'}$, so we can proceed as before, ignoring these $\Theta(k) = \Theta(1)$ normalization factors. From now on, we can proceed exactly as in the proof of Lemma~\ref{first-step-works}: first, we can use $\bm{u}^*$ to effectively proceed with the recursive calls to the sub-problems. Let $(\mathcal{S}',k'',f',\gamma')$ be the input of one of these sub-problems. In the exact same way of Lemma~\ref{first-step-works}, we get that $\|Q_{k''}^{\mathcal{S}',\mathcal{S}'} - 2\epsilon \cdot P_{k''}^{(\mathcal{S}')^*,(\mathcal{S}')^*}\|_{\inftone} \leq f' = o(\epsilon n^2)$, where we have used a coherent notation on the sub-problem. The remaining properties follow exactly as in the proof of Lemma~\ref{first-step-works}. Notice that each recursive call comes from at most $k$ chained invocations of \recur, so all the estimates about the norms and the small probabilities (e.g., of failure of the algorithm) can be affected by a factor of $poly(k) = \Theta(1)$, which does not affect the asymptotic estimates.
\end{proof}

We can conclude that with high probability $\geq 1-o(1)$ all the recursive calls are successful and that the total number of misplaced nodes is $o(n)$, achieving the desired result.

\begin{theorem}\label{postadv-k-works}
With probability $1-o(1)$, Algorithm~\ref{alg:postadv-k} correctly classifies $n-o(n)$ vertices.
\end{theorem}

Let us analyse the running time of Algorithm~\ref{alg:postadv-k}.
Solving \sdp\ through \sdpsolve\ up to negligible error takes polynomial time. Likewise, computing an orthogonal basis of eigenvectors for $X$ up to negligible error takes polynomial time. Procedure \getthr\ takes polynomial time too, like all the remaining operations. The resulting running time is thus polynomial.
